PCOAST: A Pauli-based Quantum Circuit Optimization Framework

This paper presents the Pauli-based Circuit Optimization, Analysis, and Synthesis Toolchain (PCOAST), a framework for quantum circuit optimizations based on the commutative properties of Pauli strings. Prior work has demonstrated that commuting Clifford gates past Pauli rotations can expose opportunities for optimization in unitary circuits. PCOAST extends that approach by adapting the technique to mixed unitary and non-unitary circuits via generalized preparation and measurement nodes parameterized by Pauli strings. The result is the PCOAST graph, which enables novel optimizations based on whether a user needs to preserve the quantum state after executing the circuit, or whether they only need to preserve the measurement outcomes. Finally, the framework adapts a highly tunable greedy synthesis algorithm to implement the PCOAST graph with a given gate set. PCOAST is implemented as a set of compiler passes in the Intel Quantum SDK. In this paper, we evaluate its compilation performance against two leading quantum compilers, Qiskit and tket. We find that PCOAST reduces total gate count by 32.53% and 43.33% on average, compared to to the best performance achieved by Qiskit and tket respectively, two-qubit gates by 29.22% and 20.58%, and circuit depth by 42.02% and 51.27%.

==> src/example/ghz.tex <==

\subsection{Example---a GHZ circuit}

In the rest of this section we illustrate how the PoPR optimization works on an example circuit that implements and measures a 3-qubit GHZ state.

\begin{listing}
\begin{minted}{c++}
const int N = 3;
qbit qs[N]; cbit cs[N];

quantum_kernel void GHZ() {
    // initialize qubits
    for (int i=0; i<N; i++) {PrepZ(q[i]);}
    // prepare GHZ state
    H(q[0]);
    CNOT(q[0], q[1]); CNOT(q[1], q[2]);
    // measure qubits
    for (int i=0; i<N; i++) {
        MeasZ(q[i], c[i]);
    }
}
\end{minted}
\caption{Function that produces a GHZ circuit}
\label{lst:ghz}
\end{listing}

\begin{figure}
    \centering
\begin{quantikz}[row sep=0.1cm]
    & \gate{\PrepZ} & \gate{H} & \ctrl{1} & \qw      & \gate{\MeasZ} & \qw \\
    & \gate{\PrepZ} & \qw      & \targ{}  & \ctrl{1} & \gate{\MeasZ} & \qw \\
    & \gate{\PrepZ} & \qw      & \qw      & \targ{}  & \gate{\MeasZ} & \qw
\end{quantikz}
    \caption{The circuit corresponding to \cref{lst:ghz}.}
    \label{fig:ghz}
\end{figure}


\begin{figure*}
    \centering
% \begin{tikzpicture}[gate/.style={rectangle, draw},
%         baseline=(current bounding box.north)]
%     \node (Left0) {};
        
%     \node[gate] (Prep0) [right of=Left0]       {$\Prep{Z_0}{X_0}$};
%     \node[gate] (Prep1) [below=0.1cm of Prep0] {$\Prep{Z_1}{X_1}$};
%     \node[gate] (Prep2) [below=0.1cm of Prep1] {$\Prep{Z_2}{X_2}$};

%     \draw (Left0) -- (Prep0);
% \end{tikzpicture}
\begin{quantikz}[row sep=0.1cm, baseline=(current bounding box.north)]
    & \gate{\Prep{Z_0}{X_0}} & \qw \\
    & \gate{\Prep{Z_1}{X_1}} & \qw \\
    & \gate{\Prep{Z_2}{X_2}} & \qw
\end{quantikz}
\qquad
\begin{quantikz}[row sep=0.1cm, baseline=(current bounding box.north)]
    & \gate{H} & \ctrl{1} & \qw      & \gate{\MeasZ} & \qw \\
    & \qw      & \targ{}  & \ctrl{1} & \gate{\MeasZ} & \qw \\
    & \qw      & \qw      & \targ{}  & \gate{\MeasZ} & \qw
\end{quantikz}
    \caption{Intermediate PoPR graph and circuit corresponding to \cref{lst:ghz} (1).}
    \label{fig:ghz-1}
\end{figure*}


\begin{figure*}
    \centering
\begin{quantikz}[row sep=0.1cm, baseline=(current bounding box.north)]
    & \gate{\Prep{Z_0}{X_0}} & \gate[wires=3]{
        \begin{array}{c}
            \CNOT_{1,2} \circ \CNOT_{0,1} \circ H_0 \\ \\
            \begin{pmatrix}
                X_0 X_1 X_2 & Z_0 \\
                Z_0 Z_1     & X_1 X_2 \\
                Z_1 Z_2     & X_1
            \end{pmatrix}
        \end{array}}
        & \qw \\
    & \gate{\Prep{Z_1}{X_1}} & \qw               & \qw \\
    & \gate{\Prep{Z_2}{X_2}} & \qw               & \qw
\end{quantikz}
\qquad
\begin{quantikz}[row sep=0.1cm, baseline=(current bounding box.north)]
    & \gate{\MeasZ} & \qw \\
    & \gate{\MeasZ} & \qw \\
    & \gate{\MeasZ} & \qw
\end{quantikz}
    \caption{Intermediate PoPR graph and circuit corresponding to \cref{lst:ghz} (2).}
    \label{fig:ghz-2}
\end{figure*}


\begin{figure*}
    \centering
\begin{quantikz}[row sep=0.1cm, baseline=(current bounding box.north)]
    & \gate{\Prep{Z_0}{X_0}}
        & \gate{\Meas[c[0]]{X_0}}
        & \gate[wires=3]{
        \begin{array}{c}
            \CNOT_{1,2} \circ \CNOT_{0,1} \circ H_0 \\ \\
            \begin{pmatrix}
                X_0 X_1 X_2 & Z_0 \\
                Z_0 Z_1     & X_1 X_2 \\
                Z_1 Z_2     & X_1
            \end{pmatrix}
        \end{array}}
        & \qw \\
    & \gate{\Prep{Z_1}{X_1}} & \gate{\Meas[c[1]]{X_0 Z_1}} & \qw               & \qw \\
    & \gate{\Prep{Z_2}{X_2}} & \gate{\Meas[c[2]]{X_0 Z_1 Z_2}} & \qw               & \qw
\end{quantikz}
    \caption{Final PoPR graph and circuit corresponding to \cref{lst:ghz} (3).}
    \label{fig:ghz-3}
\end{figure*}

==> src/example/opt_ex.tex <==
\begin{figure*} 

  \centering

\begin{tabular}{c c}
  \subfloat[Reducing node support in the presence of a preparation node (top) is the equivalent of removing a control-line when the control is initialized via a preparation (bottom).]{  \label{fig:pcastopta}
    \begin{tikzpicture} 
      \node[scale=0.6] at (0,0) {
        \begin{tikzcd}[row sep=0.2cm]
          \startingpoprgate{\Prep{Z_0}{X_0}} \arrow[r] 
            &\poprgate{\Rot{Z_0 Z_1}{\theta/2}}
          \\
          &\startingpoprgate{\Rot{Z_1}{\theta/2}}
      \end{tikzcd}
      };
      
      \node at (2.25, 0) {\Large $\equiv$};
      
      \node[scale=0.6] at (3.5,0) {
        \begin{tikzcd}[row sep=0.2cm]
          \poprgate{\Prep{Z_0}{X_0}}
          \\
          \startingpoprgate{\Rot{Z_1}{\theta}}
        \end{tikzcd}
      };

      \node[scale=0.6] at (0, -1.25) {
        \begin{tikzcd}[row sep=0.2cm]
          & \gate{\PrepZ} & \octrl{1} & \qw \\
          & \qw & \gate{\RZ(\theta)} & \qw
        \end{tikzcd}
      };
      \node at (2.25, -1.25) {\Large $\equiv$};
      \node[scale=0.6] at (3.5, -1.25) {
        \begin{tikzcd}[row sep=0.2cm]
          & \gate{\PrepZ} & \qw \\ 
          & \gate{\RZ(\theta)} & \qw
        \end{tikzcd}
      };
    \end{tikzpicture}
  }

&
  
  \subfloat[Reducing the cost of the Pauli Frame in the presence of a preparation (top) is the equivalent of removing a CZ when the control line is initialized via a preparation (bottom).]{ \label{fig:pcastoptb}
    \begin{tikzpicture}
      \node[scale=0.6] at (0,0) {
        \begin{tikzcd}[row sep=0.2cm]
          \startingpoprgate{\Prep{Z_0}{X_0}} \arrow[r]
          & \startingframegate{1}{\begin{pmatrix}
              Z_0 & X_0 Z_1 \\
              Z_1 & Z_0 X_1
            \end{pmatrix}}
        \end{tikzcd}
      };

      \node at (2.25, 0) {\Large $\equiv$};
      
      \node[scale=0.6] at (4.25,0) {
        \begin{tikzcd}[row sep=0.2cm]
          \poprgate{\Prep{Z_0}{X_0}}
          & \startingframegate{1}{\begin{pmatrix}
                Z_0 & X_0 \\
                Z_1 & X_1
          \end{pmatrix}}
        \end{tikzcd}
      }; 

      \node[scale=0.6] at (1, -1.25) {
        \begin{tikzcd}[row sep=0.2cm]
          & \gate{\PrepZ} & \ctrl{1} & \qw \\
          & \qw & \ctrl{} & \qw &
        \end{tikzcd}
      };
      \node at (2.25, -1.25) {\Large $\equiv$};
      \node[scale=0.6] at (3.25, -1.25) {
        \begin{tikzcd}[row sep=0.3cm]
          & \gate{\PrepZ} & \qw \\ 
          & \qw & \qw
        \end{tikzcd}
      };
    \end{tikzpicture}
  }

\end{tabular}

  \subfloat[Sequence of transformations applied in the case a release outcome.]{ \label{fig:pcastoptc}
   \begin{tikzpicture}
     \node[scale=0.6, draw, thick, rounded corners, fill=blue!20] (g0) {
       \begin{tikzcd}[row sep=0.2cm, solid]
           &\startingpoprgate{\Meas[c_0]{Y_0 X_1 Z_2}} \arrow[rd]
         \\
         \startingpoprgate{\Prep{X_0}{Y_0}} \arrow[r] \arrow[rd] \arrow[ru]
         &\poprgate{\Rot{Z_0 Z_1}{\theta_1}} \arrow[r]
         & \startingframegate{1}{\begin{pmatrix}
                Z_0 X_1 & Z_1 \\
                Z_0 & X_0 Z_1 \\
                Z_2 & X_2
           \end{pmatrix}}
         \\
         &\startingpoprgate{\Meas[c_1]{X_0 Y_1 Z_2}} \arrow[ru]
         %\\
         %&\startingpoprgate{\Meas[c_1]{Z_2}}
       \end{tikzcd}
     };

     \node[scale=0.6, draw, thick, rounded corners, fill=blue!20] (g1) at (9, 0) {
       \begin{tikzcd}[row sep=0.2cm]
           &\startingpoprgate{\Meas[c_0]{Y_0 X_1 Z_2}} \arrow[rd]
         \\
         \poprgate{\Prep{X_0}{Y_0}} \arrow[rd] \arrow[ru]
         &
           & \startingframegate{1}{\begin{pmatrix}
                Z_0 & X_0 \\
                Z_1 & X_1 \\
                Z_2 & X_2
           \end{pmatrix}}
         \\
         &\startingpoprgate{\Meas[c_1]{X_0 Y_1 Z_2}} \arrow[ru]
       \end{tikzcd}
     };

     \node[scale=0.6, draw, thick, rounded corners, fill=blue!20] (g2) at (0, -2.5) {
       \begin{tikzcd}[row sep=0.2cm]
           & &\startingpoprgate{\Meas[c_0']{Y_0}} \arrow[rd]
         \\
         \poprgate{\Prep{X_0}{Y_0}} \arrow[r]
         & \startingframegate{1}{\begin{pmatrix}
                Z_0 X_1 & X_0 \\
                Z_1 X_0 & X_1 \\
                Z_2 & X_2
           \end{pmatrix}} \arrow[ru] \arrow[rd]
         &\startingpoprgate{\Meas[c']{Z_2}} \arrow[r]
         & \startingframegate{1}{\begin{aligned}
            &\cAssign{c_0}{c_0' + c'}; \\
            &\cAssign{c_1}{c_1' + c'}
        \end{aligned} }
         \\
         & &\startingpoprgate{\Meas[c_1']{Y_1}} \arrow[ru]
       \end{tikzcd}
     };

%     \node[scale=0.7] at (0, -10.5) {
%       \begin{tikzcd}[row sep=0.2cm]
%           & &\startingpoprgate{\Meas[c_0]{Y_0}}
%         \\
%        \poprgate{\Prep{X_0}{Y_0}} \arrow[r]
%         & \startingframegate{1}{\begin{pmatrix}
%                Y_0 & X_0 \\
%                Z_1 & X_1 \\
%                Z_2 & X_2
%           \end{pmatrix}} \arrow[ru]
%         &\startingpoprgate{\Meas[c_0 + c_1 + c_2]{Z_2}}
%         \\
%         & &\startingpoprgate{\Meas[c_2]{Y_1}}
%       \end{tikzcd}
%     };

%     \node at (0, -12.25) {\Large $\simeq (\mod c_0 \otimes c_1$) };
% prev -14
     \node[scale=0.6, draw, thick, rounded corners, fill=blue!20] (g3) at (9, -2.5) {
       \begin{tikzcd}[row sep=0.2cm]
           &\startingpoprgate{\Meas[c_0']{-Z_0}} \arrow[rd]
           & \startingframegate{1}{\begin{pmatrix}
                Z_0 & X_1 \\
                Z_1 & X_1 \\
                Z_2 & X_2
           \end{pmatrix}}
         \\
         \poprgate{\Prep{X_0}{Y_0}} \arrow[ru]
         &\startingpoprgate{\Meas[c']{Z_2}} \arrow[r]
         & \startingframegate{1}{\begin{aligned}
            &\cAssign{c_0}{c_0' + c'}; \\
            &\cAssign{c_1}{c_1' + c'}
        \end{aligned} }
         \\
         &\startingpoprgate{\Meas[c_2']{Y_1}} \arrow[ru]
       \end{tikzcd}
     };

     \path[->, line width = 0.3mm] (g0) edge node [above] {$\equiv^\hold$} (g1);
     \path[->, line width=0.3mm] (g1) edge node [above] {$\equiv^\release$} (g2);
     \path[->, line width=0.3mm] (g2) edge node [above] {$\equiv^\hold$} (g3);
     
    \end{tikzpicture}
  }

\caption{Examples of the \PCAST graph optimizations.}
  \label{fig:pcastopt}
\end{figure*}

==> src/example/running-example.tex <==

To illustrate the behavior of PoPR optimizations, we will show the optimization procedure on the example circuit shown in \cref{fig:circuit}.

\begin{figure*}
    \centering
    \begin{quantikz}[row sep=0.1cm]
    & \gate{\PrepZ}
        & \gate{\RX{\theta_1}} & \targ{}
        & \gate{\RX{\theta_2}} & \ctrl{1}
        & \gate{\RX{\theta_3}} & \gate{\MeasZ} & \qw \\
    & \gate{\PrepZ}
        & \gate{H}              & \ctrl{-1}
        & \qw                   & \targ{}
        & \qw                   & \gate{\MeasZ} & \qw
\end{quantikz}
    \caption{Example circuit.}
    \label{fig:circuit}
\end{figure*}

\begin{figure*}
\centering
\begin{tikzcd}[row sep=0.2cm]
    \vqw{1} & \poprgate{\Rot{X_0}{\theta_1}}
    \\
    \poprgate{\Prep{Z_0}{X_0}}
        & \qw
        & \framegate{\begin{pmatrix}
                Z_0 X_1 & X_0 \\
                X_1 & X_0 Z_1
            \end{pmatrix}}
        & \slice{} &
        & \gate{\RX{\theta_2}} & \ctrl{1}
        & \gate{\RX{\theta_3}} & \gate{\MeasZ} & \qw
    \\
    \poprgate{\Prep{Z_1}{X_1}}
        & \qw
        &
        & & % slice
        & \qw                   & \targ{}
        & \qw                   & \gate{\MeasZ} & \qw
\end{tikzcd}
    \caption{Example circuit (2).}
    \label{fig:circuit2}
\end{figure*}

\begin{figure*}
\centering
\begin{tikzcd}
    \vqw{1} & \poprgate{\Rot{X_0}{\theta_1}} \poprgrouping{1}{2}
            & \poprgate{\Rot{X_0}{\theta_2}} \vqw{1}
    \\
    \poprgate{\Prep{Z_0}{X_0}}
        & \qw
        & \framegate{\color{red}{\begin{pmatrix}
                Z_0 X_1 & Z_1 \\
                Z_0 & X_0 Z_1
            \end{pmatrix}}}
        & \slice{} &
        & \gate{\RX{\theta_3}} & \gate{\MeasZ} & \qw
    \\
    \poprgate{\Prep{Z_1}{X_1}}
        & \qw
        &
        & & % slice
        & \qw                   & \gate{\MeasZ} & \qw
\end{tikzcd}
    \caption{Example circuit (3).}
    \label{fig:circuit3}
\end{figure*}


\begin{figure*}
\centering
\begin{tikzcd}[row sep=0.2cm]
    \poprgate{\Prep{Z_0}{X_0}}
        & \poprgate{\Rot{X_0}{\theta_1 + \theta_2}}
        & \framegate{\begin{pmatrix}
                Z_0 X_1 & Z_1 \\
                Z_0 & X_0 Z_1
            \end{pmatrix}}
        & \slice{} &
        & \gate{\MeasZ} & \qw
    \\
    \poprgate{\Prep{Z_1}{X_1}} \poprgrouping{1}{2}
        & \poprgate{\color{red}{\Rot{Z_1}{\theta_3}}}
        &
        & & % slice
        & \gate{\MeasZ} & \qw
\end{tikzcd}
    \caption{Example circuit (4).}
    \label{fig:circuit4}
\end{figure*}


\begin{figure*}
\centering
\begin{tikzcd}[row sep=0.2cm]
    \poprgate{\Prep{Z_0}{X_0}}
        & \poprgate{\Rot{X_0}{\theta_1 + \theta_2}}
            \arrow[rd, dash]
            %\vqw{1}
        & \poprgate{\color{red}{\Meas{Z_0}}}
        & \framegate{\begin{pmatrix}
                Z_0 X_1 & Z_1 \\
                Z_0 & X_0 Z_1
            \end{pmatrix}}
    \\
    \poprgate{\Prep{Z_1}{X_1}}
        & \qw
        & \poprgate{\color{red}{\Meas{Z_0 X_1}}}
        &
\end{tikzcd}
    \caption{Example circuit (5).}
    \label{fig:circuit5}
\end{figure*}


\begin{figure*}
\centering
\begin{tikzcd}[row sep=0.2cm]
    & \gate{\PrepZ} & \gate{\RX{\theta_1 + \theta_2}} & \qw
    & \slice{} &
    \startingpoprgate{\Meas{Z_0}}
        & \framegate{\begin{pmatrix}
                Z_0 X_1 & Z_1 \\
                Z_0 & X_0 Z_1
            \end{pmatrix}}
    \\
    & \gate{\PrepZ} & \qw & \qw
    & & % slice
        \startingpoprgate{\Meas{Z_0 X_1}}
        &
\end{tikzcd}
    \caption{Example circuit (6). Synthesis Part 1.}
    \label{fig:circuit6}
\end{figure*}


\begin{figure*}
\centering
\begin{tikzcd}[row sep=0.2cm]
    & \gate{\PrepZ} & \gate{\RX{\theta_1 + \theta_2}} & \gate{\MeasZ} & \qw
    & \slice{}
    \\
    & \gate{\PrepZ} & \qw & \qw & \qw
    & & % slice
        \startingpoprgate{\Meas{Z_0 X_1}}
        &
        \poprgate{\begin{pmatrix}
                Z_0 X_1 & Z_1 \\
                Z_0 & X_0 Z_1
            \end{pmatrix}}
\end{tikzcd}
    \caption{Example circuit (7). Synthesis Part 2.}
    \label{fig:circuit7}
\end{figure*}


\begin{figure*}
\centering
\begin{tikzcd}[row sep=0.2cm]
    & \gate{\PrepZ} & \gate{\RX{\theta_1 + \theta_2}} & \gate{\MeasZ}
        & \ctrl{1} & \qw & \qw & \qw &
    & \slice{} &
        \startingframegate{\color{red}{\begin{pmatrix}
                X_1 & Z_1 \\
                Z_0 & X_0
            \end{pmatrix}}}
    \\
    & \gate{\PrepZ} & \qw & \qw & \control{} & \qw
         & \gate{\MeasX} & \qw &
    & & % slice
\end{tikzcd}
    \caption{Example circuit (8). Synthesis Part 3.}
    \label{fig:circuit8}
\end{figure*}


\begin{figure*}
\centering
\begin{tikzcd}[row sep=0.2cm]
    & \gate{\PrepZ} & \gate{\RX{\theta_1 + \theta_2}} & \gate{\MeasZ}
        & \ctrl{1} & \qw & \qw & \qw &  \qw & \swap{1} & \qw
    \\
    & \gate{\PrepZ} & \qw & \qw & \control{} & \qw
        & \gate{\MeasX} & \gate{H} & \qw & \targX{} & \qw
\end{tikzcd}
    \caption{Example circuit (9). Synthesis Part 4.}
    \label{fig:circuit9}
\end{figure*}

%

==> src/outdated/cqstate.tex <==
\subsection{Classical-quantum states}


In particular, preparation and measurement gates act probabilistically on quantum states. Because probability distributions can be difficult to work with, \emph{density matrices} are often used instead to represent a probability distribution over quantum states as a matrix, in which case the behavior of circuits can be described as deterministic functions over density matrices. Density matrices are $2^n \times 2^n$ complex matrices $\rho$ with trace $1$~\cite{nielsen2002quantum}. A density matrix is called a pure state if it can be written as the outer product of two state vectors $\ket{\phi}\bra{\phi}$; otherwise it is called a mixed state, and can always be written as a weighted sum of pure states.

However, density matrices lose some information when describing the behavior of mixed classical and quantum programs; namely the classical values corresponding to each branch of the probability distribution. Following \citet{feng2021quantum} and \citet{selinger2004towards}, instead of density matrices directly, we use a \emph{classical-quantum state} or cq-state, written $\bigoplus_i \cqstate{\sigma_i}{\rho_i}$: the disjoint sum of partial density matrices $\rho_i$, whose traces are between 0 and 1, paired with the classical states $\sigma_i$ they correspond to.
Here, classical states are assignments of boolean values $b$ to classical variables $c$:
\begin{align}
    \sigma &::= \cdot \mid c \mapsto b \mid \sigma, \sigma'
\end{align}
The sum of all the partial density matrices $\rho_i$ in a cq-state should themselves be a full density matrix.

When it is clear from context, we sometimes write $\rho$ for the singleton cq-state $\cqstate{\cdot}{\rho}$, and $\sigma$ for $\cqstate{\sigma}{I}$.

As an example, the cq-state obtained from executing the circuit $\PrepZ(0); H(0); c=\MeasZ(0)$ is
\begin{align}
    \cqstate{c \mapsto 0}{\frac{1}{2}\ket{0}\bra{0}}
    \oplus
    \cqstate{c \mapsto 1}{\frac{1}{2}\ket{1}\bra{1}}.
\end{align}

Note that in the state $\bigoplus_i \cqstate{\sigma_i}{\rho_i}$, we assume that $\sigma_i \neq \sigma_j$ for each $i \neq j$; if they were equal, they would be reduced to
\begin{align}
    \cqstate{\sigma}{\rho_1} \oplus \cqstate{\sigma}{\rho_2}
    &= \cqstate{\sigma}{\rho_1 + \rho_2}.
\end{align}

In this paper, while measurement gates affect the output classical part of a cq-state, no gates depend on the classical input part of a cq-state. As a result, the semantics of all gates can be described as functions $f$ from density matrices $\rho$ to cq-states, and we can lift these to $\lift{f} : \CQSTATE \rightarrow \CQSTATE$ as follows:
\begin{align}
    \lift{f}\left( \bigoplus_i \cqstate{\sigma_i}{\rho_i} \right)
    &= \bigoplus_i \bigoplus_{j} \cqstate{\sigma_i, \sigma_j'}{\rho_j'}
\end{align}
where $f(\rho_i) = \bigoplus_j \cqstate{\sigma_j'}{\rho_j'}$.
We can also defined multiplication and scaling of cq-states in a straightforward way.
\begin{ExtendedVersion}
\begin{align}
    \left(\bigoplus_i \cqstate{\sigma_i} {\rho_i}\right)
    \cdot
    \left(\bigoplus_j \cqstate{\sigma_j'} {\rho_j'}\right)
    &= \bigoplus_i \bigoplus_j \cqstate{\sigma_i,\sigma_j'}{\rho_i \rho_j'} \\
    \alpha \bigoplus_i \cqstate{\sigma_i}{\rho_i}
    &= \bigoplus_i \cqstate{\sigma_i}{\alpha \rho_i}
\end{align}
\end{ExtendedVersion}


==> src/outdated/intro-plus-related-work.tex <==
Quantum circuit optimizations address an important challenge in the design of efficient quantum computing systems by reducing the number of operations required to execute quantum algorithms~\citep{chong2017programming}. In this paper, we describe a novel optimization framework called \PCAST, a Pauli-based Circuit Optimization, Analysis, and Synthesis Toolchain, which successfully reduces the number of gates in our benchmarks by an average of \todo{average} over the top competitors competitors.

Quantum circuit optimizations fall in two main classes: local, peephole-style optimizations~\todo{cite}, where local patterns of gates are replaced by other patterns; and global optimizations, where circuits are converted to an intermediate mathematical structure that highlights some semantic equivalence, simplified according to the rules of that structure, and synthesized back into a circuit that could be significantly different from the original. While peephole optimizations can be effective for recognizing common, simple patterns, including between unitary and non-unitary gates, they tend to miss richer opportunities for optimizations, both because they only look locally at neighboring gates, and because of the number and complexity of patterns needed to identify such opportunities.

Recently, a class of global optimizations based on Pauli rotations have proved successful in reducing gate count for unitary circuits beyond the reach of more traditional local peephole optimizations~\citep{Zhang2019,cowtan2019phase,Schmitz2021}. These optimizations take advantage of the fact that unitary circuits can be decomposed into Clifford gates (generated by the Hadamard gate $H$, the phase gate $S$ and the controlled-not gate $\CNOT$); and non-Clifford gates, which can all be represented by single-qubit Pauli rotations $\Rot{P}{\theta}=e^{-i \theta/2 P}$, where $P$ is one the Pauli matrices $X$, $Y$, or $Z$. Because Clifford unitaries $U$ always map Paulis to Paulis by conjugation (meaning $U P U^\dagger$ is always a Pauli for any Pauli $P$), it is possible to push Cliffords past the non-Clifford Pauli rotations $\Rot{P}{\theta}$ to produce a new rotation $\Rot{U P U^\dagger}{\theta}$. Doing so can expose the fact that some rotations can be merged~\citep{Zhang2019}, reducing the number of gates required in the final circuit, even if the original gates did not appear directly next to each other in the original circuit. The implementation of Pauli gadgets (the equivalent of Pauli rotations) in the \tket compiler~\citep{Sivarajah_2021_tket} has been shown to reduce both the number of 2-qubit entangling gates, relevant for Noisy Intermediate Scale Quantum (NISQ) workflows, and single-qubit non-Clifford gates, relevant for fault-tolerant workflows~\citep{cowtan2019phase}.

These optimizations are quite powerful, but they fall short in two main ways. First, they focus on unitary circuits, so equivalences enabled by non-unitary operations like preparations and measurements are not taken into account. For example, if a $Z$ rotation occurs on a qubit that was prepared in a $Z$ state, that rotation can be eliminated. Incorporating non-unitary gates enables several interesting optimizations, such as the ability to drop all unitary gates after measurement, including those pushed via the above optimization, when coherence on the quantum device doesn't need to be preserved after measurement. Second, while optimizations reduce the number of rotations and put an upper bound on the size of the resulting circuit, the number of two-qubit gates required can be expensive if we choose to synthesize the rotations in the wrong order. \citet{Schmitz2021} and \citet{li2022paulihedral} both explore synthesis in the context of Hamiltonian simulation, with the goal of automatically synthesizing a Hamiltonian, described as a product of Pauli rotations, into a circuit with a designated gateset. In particular, \citeauthor{Schmitz2021} describes a greedy search algorithm  that reduces this search problem to a variation of the traveling salesman problem~\citep{Schmitz2021}.

\input{src/example/compact-example}

In this paper, we show that by addressing these deficits, Pauli strings can be used not only as a standalone optimization pass, but as a cohesive optimization framework, which we call \PCAST. As an example, consider the workflow in \cref{fig:demo}. The circuit in \cref{fig:demo-circuit} is converted into a pair of a graph, called a \PCAST graph, and a Pauli frame, representing a Clifford circuit, as shown in \cref{fig:demo-graph}. The graph highlights the commutativity of rotation nodes in relation to each other---if there is no dependency between two nodes, they commute with each other. In addition to the unitary Pauli rotations, our \PCAST graph contains non-unitary gates---preparation and measurement---that are parameterized by Pauli rotations and are subject to the same commutativity rules as rotations. To represent Cliffords, we use a compact representation as Pauli frames, otherwise known as Pauli tableaus~\citep{Aaronson2004}, which emphasizes the behavior of the Clifford on Pauli arguments (presented in \cref{sec:frame}. A summary of different types of nodes is shown in \cref{fig:nodesCategories}.

\begin{figure}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tikzpicture}
        \node[align=center, draw, rectangle, rounded corners] (pauli) at (0.5, 0.25) {Paulis \\ $X_0 Z_1 Y_3$ };
        
        \node[align=center, draw, rectangle, rounded corners] (frames) at (2.5, 0.25) {Pauli frames \\ $F : \Pauli \rightarrow \Pauli$ };

        \node[align=center] (clifford) at (1.75, 1.0)
            {Clifford gates};
        \draw[blue, very thick, rounded corners] (-0.5,-0.35) rectangle (3.75, 1.25);

        \node[align=center, draw, rectangle, rounded corners] (rotations) at (5.5, 0.5) { Pauli rotations \\ $\Rot{P}{\theta} = e^{-i \frac{\theta}{2} P}$ };

        \node[align=center] (unitary) at (3.75, 1.5)
            {Unitary gates};
        \draw[blue, very thick, rounded corners]
            (-0.75, -0.5) rectangle (7.2, 1.75);

        \node[align=center, draw, rectangle, rounded corners] (prep)
            at (9,1.25)
            {Pauli preparations \\
            $\Prep{P_Z}{P_X}$};
        \node[align=center, draw, rectangle, rounded corners] (prep)
            at (9,0.0)
            {Pauli measurements \\
            $\Meas[c]{P}$};

        \node[align=center] (gates) at (4.75, 2.0)
            {Quantum gates};
        \draw[blue, very thick, rounded corners] (-1, -0.65) rectangle (10.75, 2.25);
    \end{tikzpicture}
    }
    \caption{Types of \PCAST nodes in relation to each other. Paulis themselves are not nodes, but are represented as Pauli frames.}
    \label{fig:nodesCategories}
\end{figure}

The addition of these non-unitary nodes enables a host of additional internal optimizations on \PCAST graphs. Users can choose between two optimization outcomes: either a \emph{hold outcome}, where the optimizations preserve the semantics of the original circuit precisely; or a \emph{release outcome}, where more aggressive optimizations can be applied as long as they produce the same measurement results. A release outcome  will drop unitary gates that can be delayed until after measurement, with the guarantee that the measurement results will always be statistically equivalent. For example, if a hold outcome is specified for \cref{fig:demo}, it will be optimized to the \PCAST graph as shown in \cref{fig:demo-optimized-graph}.

Finally, we adapt \citet{Schmitz2021}'s synthesis algorithm to determine both how to order commuting nodes, and how to decompose multi-qubit nodes using sequences of two-qubit entangling gates. The result is shown in \cref{fig:demo-optimized-circuit}. We customize the synthesis algorithm with a number of heuristics to minimize cost according to a given cost model, map into a target gateset, and reduce the number of measurements for a stabilizer search. Currently, synthesis primarily aims to minimize algorithm-level resource requirements like circuit depth. Although the design allows for customization to prioritize other search criteria, the comprehensive implications of such customization, including hardware-aware layout, routing, and scheduling, are beyond the scope of this paper.

\subsection{Related Work}

Global optimization techniques include phase polynomials~\citep{amy2018towards,nam2018automated, Meijer2020architecture}, the ZX-calculus~\citep{Kissinger2020,kissinger2020reducing}\todo{cite more}, Pauli strings~\citep{li2022paulihedral}, and Pauli rotations~\citep{Zhang2019,Schmitz2021}. They tend to outperform local optimization techniques, as the underlying mathematical structures expose opportunities for reducing gate count, especially T-count. To the best of our knowledge, our \PCAST graphs are the first example of such a technique to be able to handle mixed unitary and non-unitary circuits. \jennifer{actually, not true! \cite{borgna2021hybrid} Also Pauli fusion?~\citep{deBeaudrap2020fusion}} Most similar to \PCAST graphs is \citet{Zhang2019}'s DAG representation made up of Pauli rotations and \citet{cowtan2019phase}'s Pauli gadgets based on the ZX-calculus. Both have overlap with \cref{sec:toGraph} when restricted to unitary gates, though they don't use Pauli frames to represent Cliffords, and they do not specifically address efficient the efficient synthesis of Pauli gadgets, although they point that out as an opportunity for future work. With ZX-based optimizations in particular, it is important that optimizations keep quantum processes in a ``circuit-like'' form, as not all ZX-calculus diagrams can be easily synthesized into circuits. In contrast, for \PCAST graphs it is not important that every node is implementable as a single gate, but we build synthesis into the framework to ensure that every \PCAST graph can indeed be synthesized.

\citet{Schmitz2021} and \citet{li2022paulihedral} both address synthesis in the context of Hamiltonian simulation, with the goal of starting with a Pauli string representation of a Hamiltonian, and ending with a realizable circuit. \citet{li2022paulihedral} goes so far as to propose treating its mathematical representation Paulihedral (based on Pauli strings) as an IR, or intermediate representation, to enable hardware-aware optimization and scheduling passes. In a similar way, \PCAST graphs could too be seen as an IR for the internal optimizations in \cref{sec:opts}, although IRs are more typically text-based rather than graph-based structures. As mentioned in \cref{sec:synthesis}, \citet{Schmitz2021} is the bases of the \PCAST synthesis algorithm, extended to support non-unitary gates and custom cost functions that allow the heuristic search to be fine-tuned.

\todo{Other topics of related work? Clifford synthesis?}

\todo{RYAN: add Bqskit and other synthesis work citations}


\subsection{Contributions}

This work makes the following contributions. \cref{sec:structures} introduces the main structures of the \PCAST optimization, including Pauli frames and non-unitary gates for preparation and measurement parameterized by arbitrary Paulis. We give a semantics for all of these structures in terms of partial density matrices in a Pauli basis (\cref{sec:background}), prove the correctness of key theorems in an extended version of this paper~\extendedref.

\cref{sec:optimization} describes the three major components of the \PCAST optimization: compiling a circuit to a \PCAST graph, optimizing the graph, and synthesizing a circuit back out. Further details of the internal optimizations and proofs of correctness are given in a companion paper \companion.


We have implemented \PCAST in C++ as a sequence of compiler passes in the Intel Quantum Software Development Kit (SDK)\footnote{\todo{provide link}}~\citep{Khalate2022}, and we analyze its results in \cref{sec:results}. We compare the behavior of the \PCAST optimizations to other implementations implemented in Qiskit and \tket, and find that \todo{findings}.

Finally, in \cref{sec:related} we discuss related work, and in \cref{sec:conclusion} we conclude with a discussion of future work, including plans to adapt the synthesis algorithm to include hardware-aware optimizations such as topology and scheduling.


%\subsection{Example}
%\input{src/example/running-example}

==> src/outdated/intro.tex <==
Recently, a class of unitary quantum circuit optimizations based on Pauli rotations have proved successful in reducing gate count beyond the reach of more traditional local peephole optimizations~\citep{Zhang2019,cowtan2019phase,Schmitz2021}. These optimizations take advantage of the fact that unitary circuits can be decomposed into Clifford gates (generated by the Hadamard gate $H$, the phase gate $S$ and the controlled-not gate $\CNOT$);  and non-Clifford gates, which can all be represented by single-qubit Pauli rotations $\Rot{P}{\theta}=e^{-i \theta/2 P}$, where $P$ is one the Pauli matrices $X$, $Y$, or $Z$. Because Cliffords always map Paulis to Paulis by conjugation, it is possible to push Clifford unitaries $U$ past the non-Clifford Pauli rotations $\Rot{P}{\theta}$ to produce a new rotation $\Rot{U P U^\dagger}{\theta}$. Doing so can expose the fact that some rotations can be merged~\citep{Zhang2019}, reducing the number of gates required in the final circuit, even if the original gates did not appear directly next to each other in the original circuit. The implementation of Pauli gadgets (the equivalent of Pauli rotations) in the \tket compiler~\citep{Sivarajah_2021_tket} has been shown to reduce both the number of 2-qubit entangling gates, relevant for Noisy Intermediate Scale Quantum (NISQ) workflows, and single-qubit non-Clifford gates, relevant for fault-tolerant workflows~\citep{cowtan2019phase}.


These optimizations are quite powerful, but they fall short in two main ways. First, they focus on unitary circuits, so equivalences enabled by non-unitary operations like preparations and measurements are not taken into account. For example, if a $Z$ rotation occurs on a qubit that was prepared in a $Z$ state, that rotation can be eliminated. Incorporating non-unitary gates enables several interesting optimizations, such as the ability to drop all unitary gates after measurement, including those pushed via the above optimization, when coherence on the quantum device doesn't need to be preserved after measurement. Second, while optimizations reduce the number of rotations and put an upper bound on the size of the resulting circuit, the number of two-qubit gates required can be expensive if we choose to synthesize the rotations in the wrong order. \citet{Schmitz2021} and \citet{li2022paulihedral} both explore synthesis in the context of Hamiltonian simulation, with the goal of automatically synthesizing a Hamiltonian, described as a product of Pauli rotations, into a circuit with a designated gateset. In particular, \citeauthor{Schmitz2021} describes a greedy search algorithm  that reduces this search problem to a variation of the traveling salesman problem~\citep{Schmitz2021}.


\input{src/example/compact-example}

In this paper, we show that by addressing these deficits, Pauli strings can be used not only as a standalone optimization pass, but as a cohesive optimization framework, which we call \PCAST for a Pauli-based Circuit Analysis and Synthesis Toolchain. As an example, consider the workflow in \cref{fig:demo}. The circuit in \cref{fig:demo-circuit} is converted into a pair of a graph, called a \PCAST graph, and a Pauli frame, representing a Clifford circuit, as shown in \cref{fig:demo-graph}. The graph highlights the commutativity of rotation nodes in relation to each other---if there is no dependency between two nodes, they commute with each other. In addition to the unitary Pauli rotations, our \PCAST graph contains non-unitary gates---preparation and measurement---that are parameterized by Pauli rotations and are subject to the same commutativity rules as rotations. To represent Cliffords, we use a compact representation as Pauli frames, otherwise known as Pauli tableaus~\citep{Aaronson2004}, which elegantly emphasizes the behavior of the Clifford on Pauli arguments. A summary of different types of nodes is shown in \cref{fig:nodesCategories}.

\begin{figure}
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \begin{tikzpicture}
        %\draw[red, very thick, rounded corners](0,0) rectangle (1.5,1);
        
        \node[align=center, draw, rectangle, rounded corners] (pauli) at (0.5, 0.25) {Paulis \\ $X_0 Z_1 Y_3$ };
        
        \node[align=center, draw, rectangle, rounded corners] (frames) at (2.5, 0.25) {Pauli frames \\ $F : \Pauli \rightarrow \Pauli$ };

        \node[align=center] (clifford) at (1.75, 1.0)
            {Clifford gates};
        \draw[blue, very thick, rounded corners] (-0.5,-0.35) rectangle (3.75, 1.25);

        \node[align=center, draw, rectangle, rounded corners] (rotations) at (5.5, 0.5) { Pauli rotations \\ $\Rot{P}{\theta} = e^{-i \frac{\theta}{2} P}$ };

        \node[align=center] (unitary) at (3.75, 1.5)
            {Unitary gates};
        \draw[blue, very thick, rounded corners]
            (-0.75, -0.5) rectangle (7.2, 1.75);

        \node[align=center, draw, rectangle, rounded corners] (prep)
            at (9,1.25)
            {Pauli preparations \\
            $\Prep{P_Z}{P_X}$};
        \node[align=center, draw, rectangle, rounded corners] (prep)
            at (9,0.0)
            {Pauli measurements \\
            $\Meas[c]{P}$};

        \node[align=center] (gates) at (4.75, 2.0)
            {Quantum gates};
        \draw[blue, very thick, rounded corners] (-1, -0.65) rectangle (10.75, 2.25);
    \end{tikzpicture}
    }
    \caption{Types of \PCAST nodes in relation to each other.\jennifer{Not sure if this figure is even useful. Feedback welcome.}}
    \label{fig:nodesCategories}
\end{figure}

The addition of these non-unitary nodes enables a host of additional internal optimizations on \PCAST graphs. Users can choose between two optimization outcomes: either a \emph{hold outcome}, where the optimizations preserve the semantics of the original circuit precisely; or a \emph{release outcome}, where more aggressive optimizations can be applied as long as they produce the same measurement results. A release outcome will drop unitary gates that can be delayed until after measurement, with the guarantee that the measurement results will always be statistically equivalent. For example, if a hold outcome is specified for \cref{fig:demo}, it can be optimized to the \PCAST graph as shown in \cref{fig:demo-optimized-graph}.

Finally, we adapt \citet{Schmitz2021}'s synthesis algorithm to determine both how to order commuting nodes, and how to decompose multi-qubit nodes using sequences of two-qubit entangling gates. The result is shown in \cref{fig:demo-optimized-circuit}. We customize the synthesis algorithm with a number of heuristics to minimize cost according to a given cost model, map into a target gateset, and reduce the number of measurements for a stabilizer search. Currently, synthesis primarily aims to minimize algorithm-level resource requirements like circuit depth. Although the design allows for customization to prioritize other search criteria, the comprehensive implications of such customization, including hardware-aware layout, routing, and scheduling, are beyond the scope of this paper.

This work makes the following contributions. \cref{sec:structures} introduces the main structures of the \PCAST optimization, including Pauli frames and non-unitary gates for preparation and measurement parameterized by arbitrary Paulis. We give a semantics for all of these structures in terms of partial density matrices in a Pauli basis (\cref{sec:background}), prove the correctness of key theorems in an extended version of this paper~\extendedref.

\cref{sec:optimization} describes the three major components of the \PCAST optimization: compiling a circuit to a \PCAST graph, optimizing the graph, and synthesizing a circuit back out. Further details of the internal optimizations and proofs of correctness are given in a companion paper \companion.


%In the current Noisy Intermediate Scale Quantum (NISQ) era of quantum computing, quantum circuit optimizations play an important role in minimizing the resources required to execute or simulate quantum programs. Local peephole optimization techniques like \todo{cite} replace nearby patterns of gates with more efficient patterns, and while these are efficient to implement, they may miss potential opportunities to optimize collections of gates that are further away from each other. Global optimization techniques like \todo{cite ZX} and \todo{cite phase polynomials} have a wider reach, but focus on metrics that favor fault-tolerant quantum computing, where it is advantageous to minimize the number of T gates or other non-Clifford rotations. On many NISQ architectures, such single-qubit rotations are among the cheapest gates to implement, while two-qubit gates and measurement gates can be an order-of-magnitude more expensive.

%This paper presents a new global optimization technique we call PoPR, for Products of Pauli Rotations, which brings together and extends several techniques from the literature to achieve highly-optimized circuits for a NISQ architecture. The PoPR technique starts with representations of generalized gates parameterized by Pauli matrices $I$, $X$, $Y$, and $Z$, similar to the optimization introduced by \citet{Zhang2019}. Each of these generalized gates have simple rules that describe when they commute with each other, leading naturally to a graph representation where only non-commuting gates require dependencies, and enable optimization whereby Clifford gates can be commuted to the end of a circuit past non-Clifford rotations. Unlike \citeauthor{Zhang2019}, who only focused on unitary circuits, our PoPR graphs include preparation and measurement gates, enabling additional optimizations. In addition, PoPR uses an efficient representation of Clifford circuits as Pauli frames~\citep{Schmitz2021}, also called Pauli tableaus~\citep{Aaronson2004}, which enables the efficient synthesis of both Cliffords and non-Clifford gates as described by \citet{Schmitz2021}. The addition of the highly-tunable synthesis algorithm overcomes one limitation of \citeauthor{Zhang2019}'s technique, which is that the order of non-Pauli gates in the circuit can greatly affect the final performance of the circuit. \jennifer{Not sure about that.}

We have implemented \PCAST in C++ as a sequence of compiler passes in the Intel Quantum Software Development Kit (SDK)\footnote{\todo{provide link}}~\citep{Khalate2022}, and we analyze its results in \cref{sec:results}. We compare the behavior of the \PCAST optimizations to other implementations implemented in Qiskit and \tket, and find that \todo{findings}.

Finally, in \cref{sec:related} we discuss related work, and in \cref{sec:conclusion} we conclude with a discussion of future work, including plans to adapt the synthesis algorithm to include hardware-aware optimizations such as topology and scheduling.
 


%\subsection{Example}
%\input{src/example/running-example}

==> src/tables/counts.tex <==
\begin{table*}[]
\centering
\caption{Results for total gate count, two-qubit gates, and depth compared with Qiskit and \textbackslash{}tket}
\label{tab:gate_counts}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|ccccc|l|ccccc|l|ccccc|}
\cline{3-7} \cline{9-13} \cline{15-19}
\multicolumn{1}{l}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{5}{c|}{\textbf{Gate Count}} &
   &
  \multicolumn{5}{c|}{\textbf{2Q Gates}} &
   &
  \multicolumn{5}{c|}{\textbf{Depth}} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{Benchmark}} &
  \textbf{\# qubits} &
  \multicolumn{1}{c|}{\textbf{PoPR}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O2}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O3}} &
  \multicolumn{1}{c|}{\textbf{tket\_1}} &
  \textbf{tket\_2} &
   &
  \multicolumn{1}{c|}{\textbf{PoPR}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O2}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O3}} &
  \multicolumn{1}{c|}{\textbf{tket\_1}} &
  \textbf{tket\_2} &
   &
  \multicolumn{1}{c|}{\textbf{PoPR}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O2}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O3}} &
  \multicolumn{1}{c|}{\textbf{tket\_1}} &
  \textbf{tket\_2} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_H2\_BK}} &
  4 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}47} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}117} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}117} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}79} &
  \cellcolor[HTML]{B3DCAB}76 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}13} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}38} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F0EFBD}33} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}18} &
  \cellcolor[HTML]{9ED8A2}17 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}31} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}95} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EDEEBC}86} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}66} &
  \cellcolor[HTML]{A4D9A4}60 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_H2\_JW}} &
  4 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}58} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}195} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EEEEBD}165} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}91} &
  \cellcolor[HTML]{8AD399}81 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{94D69E}19} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}56} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E5EBBB}40} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}20} &
  \cellcolor[HTML]{00B85C}16 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}25} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}126} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E9EDBC}103} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}65} &
  \cellcolor[HTML]{8FD59B}54 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_H2\_PM}} &
  4 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}53} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}119} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFBD}106} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}72} &
  \cellcolor[HTML]{BBDDAF}71 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}15} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}38} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EAEDBC}30} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}16} &
  \cellcolor[HTML]{00B85C}15 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}25} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}99} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E0E9BA}80} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}63} &
  \cellcolor[HTML]{ABDAA8}58 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_LiH\_BK}} &
  12 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}3143} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}24985} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EDEEBD}21080} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}12017} &
  \cellcolor[HTML]{AADAA7}10786 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1308} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}8680} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EBEDBC}6834} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}3385} &
  \cellcolor[HTML]{93D59D}2858 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1157} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}18549} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E8ECBB}15111} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}9799} &
  \cellcolor[HTML]{ACDAA8}8665 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_LiH\_JW}} &
  12 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}3173} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}21239} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F9F2BF}20083} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}9471} &
  \cellcolor[HTML]{9ED8A2}8225 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1295} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}8064} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F0EFBD}6666} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}2616} &
  \cellcolor[HTML]{6FCE8D}2040 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1194} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}17027} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F1EFBD}14787} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}7654} &
  \cellcolor[HTML]{9CD7A1}6310 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_LiH\_PM}} &
  12 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}3218} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}22214} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8F2BF}20897} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}11030} &
  \cellcolor[HTML]{A6D9A6}9795 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1324} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}7640} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F5F1BE}6893} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}3092} &
  \cellcolor[HTML]{8AD499}2565 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1182} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}16131} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2F0BE}14674} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}9263} &
  \cellcolor[HTML]{A7D9A6}8021 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_BeH2\_BK}} &
  14 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}7164} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}54201} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F4F0BE}48857} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}26465} &
  \cellcolor[HTML]{ABDAA8}23834 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}3049} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}18796} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F0EFBD}15936} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}7482} &
  \cellcolor[HTML]{8ED49B}6240 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}2726} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}39889} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFBD}34861} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}21702} &
  \cellcolor[HTML]{AADAA7}19029 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_BeH2\_JW}} &
  14 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}6812} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}54113} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F9F2BF}51123} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}23684} &
  \cellcolor[HTML]{9AD7A0}19974 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}2970} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}21072} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F0EFBD}17528} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}6669} &
  \cellcolor[HTML]{6FCE8D}5044 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}2571} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}44354} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F1F0BD}38564} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}19706} &
  \cellcolor[HTML]{96D69F}15619 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_BeH2\_PM}} &
  14 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}7143} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}59164} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8F2BF}55629} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}29069} &
  \cellcolor[HTML]{A9DAA7}25923 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}3051} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}20392} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F5F1BE}18418} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}8309} &
  \cellcolor[HTML]{91D59C}6913 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}2646} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}42891} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F0BE}39019} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}24475} &
  \cellcolor[HTML]{A9DAA7}21316 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_5}} &
  5 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}68} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C9E1B4}87} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{0BBA60}69} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}104} &
  \cellcolor[HTML]{C6E0B4}86 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}26} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}26} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}20} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}26} &
  \cellcolor[HTML]{00B85C}20 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}31} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}48} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{74CF8F}41} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}55} &
  \cellcolor[HTML]{CEE2B5}49 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_10}} &
  10 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}262} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}334} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{4AC77D}289} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}416} &
  \cellcolor[HTML]{DFE9B9}371 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}112} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}105} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}90} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}105} &
  \cellcolor[HTML]{00B85C}90 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}81} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}103} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{87D397}96} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}120} &
  \cellcolor[HTML]{EAEDBC}114 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_20}} &
  20 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}922} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}1269} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{92D59D}1179} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1631} &
  \cellcolor[HTML]{F0EFBD}1541 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}440} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}410} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}380} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}410} &
  \cellcolor[HTML]{00B85C}380 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}270} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{1FBE69}212} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}206} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D3E4B7}250} &
  \cellcolor[HTML]{C6E0B4}244 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_30}} &
  30 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}2281} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}2804} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{88D398}2642} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}3646} &
  \cellcolor[HTML]{F2F0BE}3466 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1119} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}915} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}858} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}915} &
  \cellcolor[HTML]{00B85C}858 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}491} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{14BC65}322} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}316} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C8E1B4}380} &
  \cellcolor[HTML]{C6E0B4}374 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_50}} &
  50 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{35C273}6348} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}7674} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}5862} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}9236} &
  \cellcolor[HTML]{C6E0B4}7666 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}3282} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D2E4B6}2525} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1898} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}2315} &
  \cellcolor[HTML]{00B85C}1898 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1324} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{0CBA61}542} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}536} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}640} &
  \cellcolor[HTML]{C6E0B4}634 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_5}} &
  5 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}37} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}52} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}52} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}62} &
  \cellcolor[HTML]{FFF5C1}62 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}13} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}13} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}13} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}13} &
  \cellcolor[HTML]{FFF5C1}13 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}6} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}35} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}35} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}44} &
  \cellcolor[HTML]{FFF5C1}44 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_10}} &
  10 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}162} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}187} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}187} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}230} &
  \cellcolor[HTML]{FFF5C1}230 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}56} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}49} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}49} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}49} &
  \cellcolor[HTML]{00B85C}49 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}11} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}94} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}94} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}124} &
  \cellcolor[HTML]{FFF5C1}124 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_30}} &
  30 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}530} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}637} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}637} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}790} &
  \cellcolor[HTML]{FFF5C1}790 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}185} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}169} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}169} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}169} &
  \cellcolor[HTML]{00B85C}169 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}26} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}274} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}274} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}364} &
  \cellcolor[HTML]{FFF5C1}364 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_80}} &
  80 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1545} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}1762} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}1762} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}2190} &
  \cellcolor[HTML]{FFF5C1}2190 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}559} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}469} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}469} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}469} &
  \cellcolor[HTML]{00B85C}469 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}63} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}721} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}721} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}960} &
  \cellcolor[HTML]{FFF5C1}960 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_100}} &
  100 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1936} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}2212} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}2212} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}2750} &
  \cellcolor[HTML]{FFF5C1}2750 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}695} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}589} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}589} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}589} &
  \cellcolor[HTML]{00B85C}589 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}78} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}901} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}901} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1200} &
  \cellcolor[HTML]{FFF5C1}1200 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_5\_linear\_20}} &
  5 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}341} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}326} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}326} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}345} &
  \cellcolor[HTML]{FFF5C1}345 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}93} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}80} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}80} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}80} &
  \cellcolor[HTML]{00B85C}80 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}114} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}106} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}106} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}106} &
  \cellcolor[HTML]{00B85C}106 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_5\_circular\_20}} &
  5 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}473} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}405} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}405} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}405} &
  \cellcolor[HTML]{00B85C}405 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}184} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}100} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}100} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}100} &
  \cellcolor[HTML]{00B85C}100 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}221} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}222} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}222} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}222} &
  \cellcolor[HTML]{FFF5C1}222 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_5\_full\_20}} &
  5 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}326} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}446} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}446} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}705} &
  \cellcolor[HTML]{FFF5C1}705 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}85} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}200} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}200} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}200} &
  \cellcolor[HTML]{FFF5C1}200 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}111} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}144} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}144} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}264} &
  \cellcolor[HTML]{FFF5C1}264 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_10\_linear\_40}} &
  10 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1591} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1451} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1451} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}1490} &
  \cellcolor[HTML]{C6E0B4}1490 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}480} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}360} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}360} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}360} &
  \cellcolor[HTML]{00B85C}360 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}277} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}216} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}216} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}216} &
  \cellcolor[HTML]{00B85C}216 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_10\_circular\_40}} &
  10 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}4348} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1610} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1610} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1610} &
  \cellcolor[HTML]{00B85C}1610 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1749} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}400} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}400} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}400} &
  \cellcolor[HTML]{00B85C}400 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}924} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}842} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}842} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}842} &
  \cellcolor[HTML]{00B85C}842 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_10\_full\_40}} &
  10 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1592} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}2891} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}2891} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}5810} &
  \cellcolor[HTML]{FFF5C1}5810 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}476} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1800} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1800} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1800} &
  \cellcolor[HTML]{FFF5C1}1800 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}275} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}489} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}489} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1129} &
  \cellcolor[HTML]{FFF5C1}1129 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_20\_linear\_50}} &
  20 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}4065} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}3821} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}3821} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}3870} &
  \cellcolor[HTML]{C6E0B4}3870 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1152} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}950} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}950} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}950} &
  \cellcolor[HTML]{00B85C}950 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}401} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}286} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}286} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}286} &
  \cellcolor[HTML]{00B85C}286 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_20\_circular\_50}} &
  20 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}20533} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}4020} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}4020} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}4020} &
  \cellcolor[HTML]{00B85C}4020 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}9048} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1000} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1000} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1000} &
  \cellcolor[HTML]{00B85C}1000 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}2207} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}2052} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}2052} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}2052} &
  \cellcolor[HTML]{00B85C}2052 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_20\_full\_50}} &
  20 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}4063} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}12371} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}12371} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}29520} &
  \cellcolor[HTML]{FFF5C1}29520 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1147} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}9500} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}9500} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}9500} &
  \cellcolor[HTML]{FFF5C1}9500 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}401} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}1119} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}1119} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}2919} &
  \cellcolor[HTML]{FFF5C1}2919 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_6\_0\_3}} &
  6 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}98} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}85} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{3CC477}89} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}108} &
  \cellcolor[HTML]{FFF5C1}108 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}23} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}24} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}24} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}24} &
  \cellcolor[HTML]{FFF5C1}24 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}36} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}37} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}37} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}50} &
  \cellcolor[HTML]{FFF5C1}50 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_6\_0\_6}} &
  6 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}97} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}93} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}93} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}122} &
  \cellcolor[HTML]{FFF5C1}122 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}25} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}28} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}28} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}28} &
  \cellcolor[HTML]{FFF5C1}28 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}37} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}51} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}51} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}76} &
  \cellcolor[HTML]{FFF5C1}76 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_17\_0\_3}} &
  17 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}432} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}406} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}406} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}586} &
  \cellcolor[HTML]{FFF5C1}586 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}148} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}148} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}148} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}148} &
  \cellcolor[HTML]{FFF5C1}148 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}90} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}81} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}81} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}114} &
  \cellcolor[HTML]{FFF5C1}114 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_17\_0\_6}} &
  17 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}731} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}761} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}761} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1202} &
  \cellcolor[HTML]{FFF5C1}1202 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}253} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}324} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}324} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}324} &
  \cellcolor[HTML]{FFF5C1}324 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}128} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}161} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}161} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}247} &
  \cellcolor[HTML]{FFF5C1}247 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_28\_0\_3}} &
  28 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}1007} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}952} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}952} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1456} &
  \cellcolor[HTML]{FFF5C1}1456 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}356} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}384} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}384} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}384} &
  \cellcolor[HTML]{FFF5C1}384 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}151} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}156} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}156} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}225} &
  \cellcolor[HTML]{FFF5C1}225 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_28\_0\_6}} &
  28 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1746} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}1870} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}1870} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}3052} &
  \cellcolor[HTML]{FFF5C1}3052 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}660} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}840} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}840} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}840} &
  \cellcolor[HTML]{FFF5C1}840 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}248} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}278} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}278} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}423} &
  \cellcolor[HTML]{FFF5C1}423 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_40\_0\_3}} &
  40 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}2169} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}2035} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}2035} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}3254} &
  \cellcolor[HTML]{FFF5C1}3254 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}865} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}884} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}884} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}884} &
  \cellcolor[HTML]{FFF5C1}884 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}251} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}279} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}279} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}418} &
  \cellcolor[HTML]{FFF5C1}418 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_40\_0\_6}} &
  40 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}3456} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}3876} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}3876} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}6460} &
  \cellcolor[HTML]{FFF5C1}6460 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}1361} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1800} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1800} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}1800} &
  \cellcolor[HTML]{FFF5C1}1800 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}413} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}418} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C6E0B4}418} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFF5C1}629} &
  \cellcolor[HTML]{FFF5C1}629 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\end{tabular}%
}
\end{table*}

==> src/tables/counts_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|ccccc|l|ccccc|l|ccccc|}
\cline{3-7} \cline{9-13} \cline{15-19}
\multicolumn{1}{l}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{5}{c|}{\textbf{Gate Count}} &
   &
  \multicolumn{5}{c|}{\textbf{2Q Gates}} &
   &
  \multicolumn{5}{c|}{\textbf{Depth}} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{Benchmark}} &
  \textbf{\# qubits} &
  \multicolumn{1}{c|}{\textbf{PoPR}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O2}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O3}} &
  \multicolumn{1}{c|}{\textbf{tket\_1}} &
  \textbf{tket\_2} &
   &
  \multicolumn{1}{c|}{\textbf{PoPR}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O2}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O3}} &
  \multicolumn{1}{c|}{\textbf{tket\_1}} &
  \textbf{tket\_2} &
   &
  \multicolumn{1}{c|}{\textbf{PoPR}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O2}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O3}} &
  \multicolumn{1}{c|}{\textbf{tket\_1}} &
  \textbf{tket\_2} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_H2\_BK}} &
  4 &
  \multicolumn{1}{c|}{\textbf{47}} &
  \multicolumn{1}{c|}{117} &
  \multicolumn{1}{c|}{117} &
  \multicolumn{1}{c|}{79} &
  76 &
   &
  \multicolumn{1}{c|}{\textbf{13}} &
  \multicolumn{1}{c|}{38} &
  \multicolumn{1}{c|}{33} &
  \multicolumn{1}{c|}{18} &
  17 &
   &
  \multicolumn{1}{c|}{\textbf{31}} &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{86} &
  \multicolumn{1}{c|}{66} &
  60 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_H2\_JW}} &
  4 &
  \multicolumn{1}{c|}{\textbf{58}} &
  \multicolumn{1}{c|}{195} &
  \multicolumn{1}{c|}{165} &
  \multicolumn{1}{c|}{91} &
  81 &
   &
  \multicolumn{1}{c|}{19} &
  \multicolumn{1}{c|}{56} &
  \multicolumn{1}{c|}{40} &
  \multicolumn{1}{c|}{20} &
  \textbf{16} &
   &
  \multicolumn{1}{c|}{\textbf{25}} &
  \multicolumn{1}{c|}{126} &
  \multicolumn{1}{c|}{103} &
  \multicolumn{1}{c|}{65} &
  54 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_H2\_PM}} &
  4 &
  \multicolumn{1}{c|}{\textbf{53}} &
  \multicolumn{1}{c|}{119} &
  \multicolumn{1}{c|}{106} &
  \multicolumn{1}{c|}{72} &
  71 &
   &
  \multicolumn{1}{c|}{\textbf{15}} &
  \multicolumn{1}{c|}{38} &
  \multicolumn{1}{c|}{30} &
  \multicolumn{1}{c|}{16} &
  \textbf{15} &
   &
  \multicolumn{1}{c|}{\textbf{25}} &
  \multicolumn{1}{c|}{99} &
  \multicolumn{1}{c|}{80} &
  \multicolumn{1}{c|}{63} &
  58 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_LiH\_BK}} &
  12 &
  \multicolumn{1}{c|}{\textbf{3143}} &
  \multicolumn{1}{c|}{24985} &
  \multicolumn{1}{c|}{21080} &
  \multicolumn{1}{c|}{12017} &
  10786 &
   &
  \multicolumn{1}{c|}{\textbf{1308}} &
  \multicolumn{1}{c|}{8680} &
  \multicolumn{1}{c|}{6834} &
  \multicolumn{1}{c|}{3385} &
  2858 &
   &
  \multicolumn{1}{c|}{\textbf{1157}} &
  \multicolumn{1}{c|}{18549} &
  \multicolumn{1}{c|}{15111} &
  \multicolumn{1}{c|}{9799} &
  8665 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_LiH\_JW}} &
  12 &
  \multicolumn{1}{c|}{\textbf{3173}} &
  \multicolumn{1}{c|}{21239} &
  \multicolumn{1}{c|}{20083} &
  \multicolumn{1}{c|}{9471} &
  8225 &
   &
  \multicolumn{1}{c|}{\textbf{1295}} &
  \multicolumn{1}{c|}{8064} &
  \multicolumn{1}{c|}{6666} &
  \multicolumn{1}{c|}{2616} &
  2040 &
   &
  \multicolumn{1}{c|}{\textbf{1194}} &
  \multicolumn{1}{c|}{17027} &
  \multicolumn{1}{c|}{14787} &
  \multicolumn{1}{c|}{7654} &
  6310 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_LiH\_PM}} &
  12 &
  \multicolumn{1}{c|}{\textbf{3218}} &
  \multicolumn{1}{c|}{22214} &
  \multicolumn{1}{c|}{20897} &
  \multicolumn{1}{c|}{11030} &
  9795 &
   &
  \multicolumn{1}{c|}{\textbf{1324}} &
  \multicolumn{1}{c|}{7640} &
  \multicolumn{1}{c|}{6893} &
  \multicolumn{1}{c|}{3092} &
  2565 &
   &
  \multicolumn{1}{c|}{\textbf{1182}} &
  \multicolumn{1}{c|}{16131} &
  \multicolumn{1}{c|}{14674} &
  \multicolumn{1}{c|}{9263} &
  8021 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_BeH2\_BK}} &
  14 &
  \multicolumn{1}{c|}{\textbf{7164}} &
  \multicolumn{1}{c|}{54201} &
  \multicolumn{1}{c|}{48857} &
  \multicolumn{1}{c|}{26465} &
  23834 &
   &
  \multicolumn{1}{c|}{\textbf{3049}} &
  \multicolumn{1}{c|}{18796} &
  \multicolumn{1}{c|}{15936} &
  \multicolumn{1}{c|}{7482} &
  6240 &
   &
  \multicolumn{1}{c|}{\textbf{2726}} &
  \multicolumn{1}{c|}{39889} &
  \multicolumn{1}{c|}{34861} &
  \multicolumn{1}{c|}{21702} &
  19029 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_BeH2\_JW}} &
  14 &
  \multicolumn{1}{c|}{\textbf{6812}} &
  \multicolumn{1}{c|}{54113} &
  \multicolumn{1}{c|}{51123} &
  \multicolumn{1}{c|}{23684} &
  19974 &
   &
  \multicolumn{1}{c|}{\textbf{2970}} &
  \multicolumn{1}{c|}{21072} &
  \multicolumn{1}{c|}{17528} &
  \multicolumn{1}{c|}{6669} &
  5044 &
   &
  \multicolumn{1}{c|}{\textbf{2571}} &
  \multicolumn{1}{c|}{44354} &
  \multicolumn{1}{c|}{38564} &
  \multicolumn{1}{c|}{19706} &
  15619 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_BeH2\_PM}} &
  14 &
  \multicolumn{1}{c|}{\textbf{7143}} &
  \multicolumn{1}{c|}{59164} &
  \multicolumn{1}{c|}{55629} &
  \multicolumn{1}{c|}{29069} &
  25923 &
   &
  \multicolumn{1}{c|}{\textbf{3051}} &
  \multicolumn{1}{c|}{20392} &
  \multicolumn{1}{c|}{18418} &
  \multicolumn{1}{c|}{8309} &
  6913 &
   &
  \multicolumn{1}{c|}{\textbf{2646}} &
  \multicolumn{1}{c|}{42891} &
  \multicolumn{1}{c|}{39019} &
  \multicolumn{1}{c|}{24475} &
  21316 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_5}} &
  5 &
  \multicolumn{1}{c|}{\textbf{68}} &
  \multicolumn{1}{c|}{87} &
  \multicolumn{1}{c|}{69} &
  \multicolumn{1}{c|}{104} &
  86 &
   &
  \multicolumn{1}{c|}{26} &
  \multicolumn{1}{c|}{26} &
  \multicolumn{1}{c|}{\textbf{20}} &
  \multicolumn{1}{c|}{26} &
  \textbf{20} &
   &
  \multicolumn{1}{c|}{\textbf{31}} &
  \multicolumn{1}{c|}{48} &
  \multicolumn{1}{c|}{41} &
  \multicolumn{1}{c|}{55} &
  49 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_10}} &
  10 &
  \multicolumn{1}{c|}{\textbf{262}} &
  \multicolumn{1}{c|}{334} &
  \multicolumn{1}{c|}{289} &
  \multicolumn{1}{c|}{416} &
  371 &
   &
  \multicolumn{1}{c|}{112} &
  \multicolumn{1}{c|}{105} &
  \multicolumn{1}{c|}{\textbf{90}} &
  \multicolumn{1}{c|}{105} &
  \textbf{90} &
   &
  \multicolumn{1}{c|}{\textbf{81}} &
  \multicolumn{1}{c|}{103} &
  \multicolumn{1}{c|}{96} &
  \multicolumn{1}{c|}{120} &
  114 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_20}} &
  20 &
  \multicolumn{1}{c|}{\textbf{922}} &
  \multicolumn{1}{c|}{1269} &
  \multicolumn{1}{c|}{1179} &
  \multicolumn{1}{c|}{1631} &
  1541 &
   &
  \multicolumn{1}{c|}{440} &
  \multicolumn{1}{c|}{410} &
  \multicolumn{1}{c|}{\textbf{380}} &
  \multicolumn{1}{c|}{410} &
  \textbf{380} &
   &
  \multicolumn{1}{c|}{270} &
  \multicolumn{1}{c|}{212} &
  \multicolumn{1}{c|}{\textbf{206}} &
  \multicolumn{1}{c|}{250} &
  244 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_30}} &
  30 &
  \multicolumn{1}{c|}{\textbf{2281}} &
  \multicolumn{1}{c|}{2804} &
  \multicolumn{1}{c|}{2642} &
  \multicolumn{1}{c|}{3646} &
  3466 &
   &
  \multicolumn{1}{c|}{1119} &
  \multicolumn{1}{c|}{915} &
  \multicolumn{1}{c|}{\textbf{858}} &
  \multicolumn{1}{c|}{915} &
  \textbf{858} &
   &
  \multicolumn{1}{c|}{491} &
  \multicolumn{1}{c|}{322} &
  \multicolumn{1}{c|}{\textbf{316}} &
  \multicolumn{1}{c|}{380} &
  374 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_50}} &
  50 &
  \multicolumn{1}{c|}{6348} &
  \multicolumn{1}{c|}{7674} &
  \multicolumn{1}{c|}{\textbf{5862}} &
  \multicolumn{1}{c|}{9236} &
  7666 &
   &
  \multicolumn{1}{c|}{3282} &
  \multicolumn{1}{c|}{2525} &
  \multicolumn{1}{c|}{\textbf{1898}} &
  \multicolumn{1}{c|}{2315} &
  \textbf{1898} &
   &
  \multicolumn{1}{c|}{1324} &
  \multicolumn{1}{c|}{542} &
  \multicolumn{1}{c|}{\textbf{536}} &
  \multicolumn{1}{c|}{640} &
  634 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_5}} &
  5 &
  \multicolumn{1}{c|}{\textbf{37}} &
  \multicolumn{1}{c|}{52} &
  \multicolumn{1}{c|}{52} &
  \multicolumn{1}{c|}{62} &
  62 &
   &
  \multicolumn{1}{c|}{\textbf{13}} &
  \multicolumn{1}{c|}{\textbf{13}} &
  \multicolumn{1}{c|}{\textbf{13}} &
  \multicolumn{1}{c|}{\textbf{13}} &
  \textbf{13} &
   &
  \multicolumn{1}{c|}{\textbf{6}} &
  \multicolumn{1}{c|}{35} &
  \multicolumn{1}{c|}{35} &
  \multicolumn{1}{c|}{44} &
  44 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_10}} &
  10 &
  \multicolumn{1}{c|}{\textbf{162}} &
  \multicolumn{1}{c|}{187} &
  \multicolumn{1}{c|}{187} &
  \multicolumn{1}{c|}{230} &
  230 &
   &
  \multicolumn{1}{c|}{56} &
  \multicolumn{1}{c|}{\textbf{49}} &
  \multicolumn{1}{c|}{\textbf{49}} &
  \multicolumn{1}{c|}{\textbf{49}} &
  \textbf{49} &
   &
  \multicolumn{1}{c|}{\textbf{11}} &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{124} &
  124 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_30}} &
  30 &
  \multicolumn{1}{c|}{\textbf{530}} &
  \multicolumn{1}{c|}{637} &
  \multicolumn{1}{c|}{637} &
  \multicolumn{1}{c|}{790} &
  790 &
   &
  \multicolumn{1}{c|}{185} &
  \multicolumn{1}{c|}{\textbf{169}} &
  \multicolumn{1}{c|}{\textbf{169}} &
  \multicolumn{1}{c|}{\textbf{169}} &
  \textbf{169} &
   &
  \multicolumn{1}{c|}{\textbf{26}} &
  \multicolumn{1}{c|}{274} &
  \multicolumn{1}{c|}{274} &
  \multicolumn{1}{c|}{364} &
  364 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_80}} &
  80 &
  \multicolumn{1}{c|}{\textbf{1545}} &
  \multicolumn{1}{c|}{1762} &
  \multicolumn{1}{c|}{1762} &
  \multicolumn{1}{c|}{2190} &
  2190 &
   &
  \multicolumn{1}{c|}{559} &
  \multicolumn{1}{c|}{\textbf{469}} &
  \multicolumn{1}{c|}{\textbf{469}} &
  \multicolumn{1}{c|}{\textbf{469}} &
  \textbf{469} &
   &
  \multicolumn{1}{c|}{\textbf{63}} &
  \multicolumn{1}{c|}{721} &
  \multicolumn{1}{c|}{721} &
  \multicolumn{1}{c|}{960} &
  960 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_100}} &
  100 &
  \multicolumn{1}{c|}{\textbf{1936}} &
  \multicolumn{1}{c|}{2212} &
  \multicolumn{1}{c|}{2212} &
  \multicolumn{1}{c|}{2750} &
  2750 &
   &
  \multicolumn{1}{c|}{695} &
  \multicolumn{1}{c|}{\textbf{589}} &
  \multicolumn{1}{c|}{\textbf{589}} &
  \multicolumn{1}{c|}{\textbf{589}} &
  \textbf{589} &
   &
  \multicolumn{1}{c|}{\textbf{78}} &
  \multicolumn{1}{c|}{901} &
  \multicolumn{1}{c|}{901} &
  \multicolumn{1}{c|}{1200} &
  1200 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_5\_linear\_20}} &
  5 &
  \multicolumn{1}{c|}{341} &
  \multicolumn{1}{c|}{\textbf{326}} &
  \multicolumn{1}{c|}{\textbf{326}} &
  \multicolumn{1}{c|}{345} &
  345 &
   &
  \multicolumn{1}{c|}{93} &
  \multicolumn{1}{c|}{\textbf{80}} &
  \multicolumn{1}{c|}{\textbf{80}} &
  \multicolumn{1}{c|}{\textbf{80}} &
  \textbf{80} &
   &
  \multicolumn{1}{c|}{114} &
  \multicolumn{1}{c|}{\textbf{106}} &
  \multicolumn{1}{c|}{\textbf{106}} &
  \multicolumn{1}{c|}{\textbf{106}} &
  \textbf{106} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_5\_circular\_20}} &
  5 &
  \multicolumn{1}{c|}{473} &
  \multicolumn{1}{c|}{\textbf{405}} &
  \multicolumn{1}{c|}{\textbf{405}} &
  \multicolumn{1}{c|}{\textbf{405}} &
  \textbf{405} &
   &
  \multicolumn{1}{c|}{184} &
  \multicolumn{1}{c|}{\textbf{100}} &
  \multicolumn{1}{c|}{\textbf{100}} &
  \multicolumn{1}{c|}{\textbf{100}} &
  \textbf{100} &
   &
  \multicolumn{1}{c|}{\textbf{221}} &
  \multicolumn{1}{c|}{222} &
  \multicolumn{1}{c|}{222} &
  \multicolumn{1}{c|}{222} &
  222 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_5\_full\_20}} &
  5 &
  \multicolumn{1}{c|}{\textbf{326}} &
  \multicolumn{1}{c|}{446} &
  \multicolumn{1}{c|}{446} &
  \multicolumn{1}{c|}{705} &
  705 &
   &
  \multicolumn{1}{c|}{\textbf{85}} &
  \multicolumn{1}{c|}{200} &
  \multicolumn{1}{c|}{200} &
  \multicolumn{1}{c|}{200} &
  200 &
   &
  \multicolumn{1}{c|}{\textbf{111}} &
  \multicolumn{1}{c|}{144} &
  \multicolumn{1}{c|}{144} &
  \multicolumn{1}{c|}{264} &
  264 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_10\_linear\_40}} &
  10 &
  \multicolumn{1}{c|}{1591} &
  \multicolumn{1}{c|}{\textbf{1451}} &
  \multicolumn{1}{c|}{\textbf{1451}} &
  \multicolumn{1}{c|}{1490} &
  1490 &
   &
  \multicolumn{1}{c|}{480} &
  \multicolumn{1}{c|}{\textbf{360}} &
  \multicolumn{1}{c|}{\textbf{360}} &
  \multicolumn{1}{c|}{\textbf{360}} &
  \textbf{360} &
   &
  \multicolumn{1}{c|}{277} &
  \multicolumn{1}{c|}{\textbf{216}} &
  \multicolumn{1}{c|}{\textbf{216}} &
  \multicolumn{1}{c|}{\textbf{216}} &
  \textbf{216} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_10\_circular\_40}} &
  10 &
  \multicolumn{1}{c|}{4348} &
  \multicolumn{1}{c|}{\textbf{1610}} &
  \multicolumn{1}{c|}{\textbf{1610}} &
  \multicolumn{1}{c|}{\textbf{1610}} &
  \textbf{1610} &
   &
  \multicolumn{1}{c|}{1749} &
  \multicolumn{1}{c|}{\textbf{400}} &
  \multicolumn{1}{c|}{\textbf{400}} &
  \multicolumn{1}{c|}{\textbf{400}} &
  \textbf{400} &
   &
  \multicolumn{1}{c|}{924} &
  \multicolumn{1}{c|}{\textbf{842}} &
  \multicolumn{1}{c|}{\textbf{842}} &
  \multicolumn{1}{c|}{\textbf{842}} &
  \textbf{842} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_10\_full\_40}} &
  10 &
  \multicolumn{1}{c|}{\textbf{1592}} &
  \multicolumn{1}{c|}{2891} &
  \multicolumn{1}{c|}{2891} &
  \multicolumn{1}{c|}{5810} &
  5810 &
   &
  \multicolumn{1}{c|}{\textbf{476}} &
  \multicolumn{1}{c|}{1800} &
  \multicolumn{1}{c|}{1800} &
  \multicolumn{1}{c|}{1800} &
  1800 &
   &
  \multicolumn{1}{c|}{\textbf{275}} &
  \multicolumn{1}{c|}{489} &
  \multicolumn{1}{c|}{489} &
  \multicolumn{1}{c|}{1129} &
  1129 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_20\_linear\_50}} &
  20 &
  \multicolumn{1}{c|}{4065} &
  \multicolumn{1}{c|}{\textbf{3821}} &
  \multicolumn{1}{c|}{\textbf{3821}} &
  \multicolumn{1}{c|}{3870} &
  3870 &
   &
  \multicolumn{1}{c|}{1152} &
  \multicolumn{1}{c|}{\textbf{950}} &
  \multicolumn{1}{c|}{\textbf{950}} &
  \multicolumn{1}{c|}{\textbf{950}} &
  \textbf{950} &
   &
  \multicolumn{1}{c|}{401} &
  \multicolumn{1}{c|}{\textbf{286}} &
  \multicolumn{1}{c|}{\textbf{286}} &
  \multicolumn{1}{c|}{\textbf{286}} &
  \textbf{286} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_20\_circular\_50}} &
  20 &
  \multicolumn{1}{c|}{20533} &
  \multicolumn{1}{c|}{\textbf{4020}} &
  \multicolumn{1}{c|}{\textbf{4020}} &
  \multicolumn{1}{c|}{\textbf{4020}} &
  \textbf{4020} &
   &
  \multicolumn{1}{c|}{9048} &
  \multicolumn{1}{c|}{\textbf{1000}} &
  \multicolumn{1}{c|}{\textbf{1000}} &
  \multicolumn{1}{c|}{\textbf{1000}} &
  \textbf{1000} &
   &
  \multicolumn{1}{c|}{2207} &
  \multicolumn{1}{c|}{\textbf{2052}} &
  \multicolumn{1}{c|}{\textbf{2052}} &
  \multicolumn{1}{c|}{\textbf{2052}} &
  \textbf{2052} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_20\_full\_50}} &
  20 &
  \multicolumn{1}{c|}{\textbf{4063}} &
  \multicolumn{1}{c|}{12371} &
  \multicolumn{1}{c|}{12371} &
  \multicolumn{1}{c|}{29520} &
  29520 &
   &
  \multicolumn{1}{c|}{\textbf{1147}} &
  \multicolumn{1}{c|}{9500} &
  \multicolumn{1}{c|}{9500} &
  \multicolumn{1}{c|}{9500} &
  9500 &
   &
  \multicolumn{1}{c|}{\textbf{401}} &
  \multicolumn{1}{c|}{1119} &
  \multicolumn{1}{c|}{1119} &
  \multicolumn{1}{c|}{2919} &
  2919 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_6\_0\_3}} &
  6 &
  \multicolumn{1}{c|}{98} &
  \multicolumn{1}{c|}{\textbf{85}} &
  \multicolumn{1}{c|}{89} &
  \multicolumn{1}{c|}{108} &
  108 &
   &
  \multicolumn{1}{c|}{\textbf{23}} &
  \multicolumn{1}{c|}{24} &
  \multicolumn{1}{c|}{24} &
  \multicolumn{1}{c|}{24} &
  24 &
   &
  \multicolumn{1}{c|}{\textbf{36}} &
  \multicolumn{1}{c|}{37} &
  \multicolumn{1}{c|}{37} &
  \multicolumn{1}{c|}{50} &
  50 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_6\_0\_6}} &
  6 &
  \multicolumn{1}{c|}{97} &
  \multicolumn{1}{c|}{\textbf{93}} &
  \multicolumn{1}{c|}{\textbf{93}} &
  \multicolumn{1}{c|}{122} &
  122 &
   &
  \multicolumn{1}{c|}{\textbf{25}} &
  \multicolumn{1}{c|}{28} &
  \multicolumn{1}{c|}{28} &
  \multicolumn{1}{c|}{28} &
  28 &
   &
  \multicolumn{1}{c|}{\textbf{37}} &
  \multicolumn{1}{c|}{51} &
  \multicolumn{1}{c|}{51} &
  \multicolumn{1}{c|}{76} &
  76 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_17\_0\_3}} &
  17 &
  \multicolumn{1}{c|}{432} &
  \multicolumn{1}{c|}{\textbf{406}} &
  \multicolumn{1}{c|}{\textbf{406}} &
  \multicolumn{1}{c|}{586} &
  586 &
   &
  \multicolumn{1}{c|}{\textbf{148}} &
  \multicolumn{1}{c|}{\textbf{148}} &
  \multicolumn{1}{c|}{\textbf{148}} &
  \multicolumn{1}{c|}{\textbf{148}} &
  \textbf{148} &
   &
  \multicolumn{1}{c|}{90} &
  \multicolumn{1}{c|}{\textbf{81}} &
  \multicolumn{1}{c|}{\textbf{81}} &
  \multicolumn{1}{c|}{114} &
  114 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_17\_0\_6}} &
  17 &
  \multicolumn{1}{c|}{\textbf{731}} &
  \multicolumn{1}{c|}{761} &
  \multicolumn{1}{c|}{761} &
  \multicolumn{1}{c|}{1202} &
  1202 &
   &
  \multicolumn{1}{c|}{\textbf{253}} &
  \multicolumn{1}{c|}{324} &
  \multicolumn{1}{c|}{324} &
  \multicolumn{1}{c|}{324} &
  324 &
   &
  \multicolumn{1}{c|}{\textbf{128}} &
  \multicolumn{1}{c|}{161} &
  \multicolumn{1}{c|}{161} &
  \multicolumn{1}{c|}{247} &
  247 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_28\_0\_3}} &
  28 &
  \multicolumn{1}{c|}{1007} &
  \multicolumn{1}{c|}{\textbf{952}} &
  \multicolumn{1}{c|}{\textbf{952}} &
  \multicolumn{1}{c|}{1456} &
  1456 &
   &
  \multicolumn{1}{c|}{\textbf{356}} &
  \multicolumn{1}{c|}{384} &
  \multicolumn{1}{c|}{384} &
  \multicolumn{1}{c|}{384} &
  384 &
   &
  \multicolumn{1}{c|}{\textbf{151}} &
  \multicolumn{1}{c|}{156} &
  \multicolumn{1}{c|}{156} &
  \multicolumn{1}{c|}{225} &
  225 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_28\_0\_6}} &
  28 &
  \multicolumn{1}{c|}{\textbf{1746}} &
  \multicolumn{1}{c|}{1870} &
  \multicolumn{1}{c|}{1870} &
  \multicolumn{1}{c|}{3052} &
  3052 &
   &
  \multicolumn{1}{c|}{\textbf{660}} &
  \multicolumn{1}{c|}{840} &
  \multicolumn{1}{c|}{840} &
  \multicolumn{1}{c|}{840} &
  840 &
   &
  \multicolumn{1}{c|}{\textbf{248}} &
  \multicolumn{1}{c|}{278} &
  \multicolumn{1}{c|}{278} &
  \multicolumn{1}{c|}{423} &
  423 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_40\_0\_3}} &
  40 &
  \multicolumn{1}{c|}{2169} &
  \multicolumn{1}{c|}{\textbf{2035}} &
  \multicolumn{1}{c|}{\textbf{2035}} &
  \multicolumn{1}{c|}{3254} &
  3254 &
   &
  \multicolumn{1}{c|}{\textbf{865}} &
  \multicolumn{1}{c|}{884} &
  \multicolumn{1}{c|}{884} &
  \multicolumn{1}{c|}{884} &
  884 &
   &
  \multicolumn{1}{c|}{\textbf{251}} &
  \multicolumn{1}{c|}{279} &
  \multicolumn{1}{c|}{279} &
  \multicolumn{1}{c|}{418} &
  418 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_40\_0\_6}} &
  40 &
  \multicolumn{1}{c|}{\textbf{3456}} &
  \multicolumn{1}{c|}{3876} &
  \multicolumn{1}{c|}{3876} &
  \multicolumn{1}{c|}{6460} &
  6460 &
   &
  \multicolumn{1}{c|}{\textbf{1361}} &
  \multicolumn{1}{c|}{1800} &
  \multicolumn{1}{c|}{1800} &
  \multicolumn{1}{c|}{1800} &
  1800 &
   &
  \multicolumn{1}{c|}{\textbf{413}} &
  \multicolumn{1}{c|}{418} &
  \multicolumn{1}{c|}{418} &
  \multicolumn{1}{c|}{629} &
  629 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\end{tabular}%
}
\end{table*}

==> src/tables/counts_v3.tex <==
\begin{table*}
\centering
\caption{Results for total gate count, two-qubit gates, and depth compared with Qiskit and \tket. The table cells' coloring indicates the range from best (green) to worst (white)}
\label{tab:gate_counts3}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|ccccc|l|ccccc|l|ccccc|}
\cline{3-7} \cline{9-13} \cline{15-19}
\multicolumn{1}{l}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{5}{c|}{\textbf{Gate Count}} &
   &
  \multicolumn{5}{c|}{\textbf{2Q Gates}} &
   &
  \multicolumn{5}{c|}{\textbf{Depth}} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{Benchmark}} &
  \textbf{\# qubits} &
  \multicolumn{1}{c|}{\textbf{PCOAST}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O2}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O3}} &
  \multicolumn{1}{c|}{\textbf{tket\_1}} &
  \textbf{tket\_2} &
   &
  \multicolumn{1}{c|}{\textbf{PCOAST}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O2}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O3}} &
  \multicolumn{1}{c|}{\textbf{tket\_1}} &
  \textbf{tket\_2} &
   &
  \multicolumn{1}{c|}{\textbf{PCOAST}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O2}} &
  \multicolumn{1}{c|}{\textbf{qiskit -O3}} &
  \multicolumn{1}{c|}{\textbf{tket\_1}} &
  \textbf{tket\_2} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_H2\_BK}} &
  4 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{47}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}117} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}117} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CEEACF}79} &
  \cellcolor[HTML]{BBE5C4}76 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{13}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}38} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F8F0}33} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{5ACE8E}18} &
  \cellcolor[HTML]{48C984}17 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{31}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}95} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F6FAF4}86} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E4F0DD}66} &
  \cellcolor[HTML]{CCE9CE}60 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_H2\_JW}} &
  4 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{58}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}195} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2F7EE}165} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{6CD298}91} &
  \cellcolor[HTML]{4BCA86}81 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{21C06E}19} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}56} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E7F2E1}40} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{2DC375}20} &
  \cellcolor[HTML]{00B85C}\textbf{16} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{25}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}126} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F1F7EE}103} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{B3E3BF}65} &
  \cellcolor[HTML]{81D7A4}54 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_H2\_PM}} &
  4 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{53}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}119} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F8F0}106} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{82D7A4}72} &
  \cellcolor[HTML]{7BD5A0}71 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{15}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}38} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EAF3E5}30} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{13BC66}16} &
  \cellcolor[HTML]{00B85C}\textbf{15} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{25}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}99} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F0F6EB}80} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}63} &
  \cellcolor[HTML]{C9E9CC}58 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_LiH\_BK}} &
  12 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{3143}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}24985} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F4F9F1}21080} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{B7E4C2}12017} &
  \cellcolor[HTML]{9EDEB4}10786 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1308}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}8680} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F0F6EC}6834} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{7FD6A2}3385} &
  \cellcolor[HTML]{5FCF90}2858 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1157}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}18549} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F8F0}15111} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E0EED9}9799} &
  \cellcolor[HTML]{C3E7C8}8665 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_LiH\_JW}} &
  12 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{3173}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}21239} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FBFCFA}20083} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{9DDEB3}9471} &
  \cellcolor[HTML]{7ED6A2}8225 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1295}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}8064} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F8EF}6666} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{58CD8D}2616} &
  \cellcolor[HTML]{31C477}2040 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1194}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}17027} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F6FAF4}14787} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{B8E4C2}7654} &
  \cellcolor[HTML]{92DBAD}6310 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_LiH\_PM}} &
  12 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{3218}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}22214} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FAFCF9}20897} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{B9E5C3}11030} &
  \cellcolor[HTML]{9CDEB3}9795 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1324}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}7640} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8FBF6}6893} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{7ED6A2}3092} &
  \cellcolor[HTML]{58CD8D}2565 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1182}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}16131} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBF7}14674} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E4F0DD}9263} &
  \cellcolor[HTML]{CEEACF}8021 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_BeH2\_BK}} &
  14 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{7164}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}54201} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8FBF6}48857} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{B9E5C3}26465} &
  \cellcolor[HTML]{A0DEB5}23834 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{3049}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}18796} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F4F9F1}15936} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{7FD6A2}7482} &
  \cellcolor[HTML]{5BCE8F}6240 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{2726}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}39889} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F7FAF4}34861} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}21702} &
  \cellcolor[HTML]{C6E8CA}19029 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_BeH2\_JW}} &
  14 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{6812}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}54113} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FBFCFA}51123} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{A1DFB5}23684} &
  \cellcolor[HTML]{7DD6A2}19974 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{2970}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}21072} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F8F0}17528} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{5CCE8F}6669} &
  \cellcolor[HTML]{33C478}5044 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{2571}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}44354} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F6FAF4}38564} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{B9E5C3}19706} &
  \cellcolor[HTML]{8DDAAA}15619 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{UCCSD\_BeH2\_PM}} &
  14 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{7143}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}59164} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FBFCF9}55629} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{BEE6C6}29069} &
  \cellcolor[HTML]{A3DFB6}25923 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{3051}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}20392} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8FBF6}18418} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{89D9A8}8309} &
  \cellcolor[HTML]{64D094}6913 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{2646}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}42891} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F9FBF7}39019} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E4F0DD}24475} &
  \cellcolor[HTML]{D1EBD0}21316 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_5}} &
  5 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{68}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E3EFDC}87} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{0CBB63}69} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}104} &
  \cellcolor[HTML]{E2EFDA}86 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}26} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}26} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{20}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}26} &
  \cellcolor[HTML]{00B85C}\textbf{20} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{31}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EEF5E9}48} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{BCE5C5}41} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}55} &
  \cellcolor[HTML]{F0F7EC}49 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_10}} &
  10 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{262}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D3EBD1}334} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{4FCB88}289} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}416} &
  \cellcolor[HTML]{EEF5E9}371 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}112} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{ECF4E7}105} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{90}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{ECF4E7}105} &
  \cellcolor[HTML]{00B85C}\textbf{90} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{81}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E5F1DE}103} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{ADE2BC}96} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}120} &
  \cellcolor[HTML]{F6FAF3}114 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_20}} &
  20 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{922}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{DDEDD7}1269} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{A3DFB7}1179} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1631} &
  \cellcolor[HTML]{F7FAF5}1541 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}440} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}410} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{380}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}410} &
  \cellcolor[HTML]{00B85C}\textbf{380} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}270} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{2AC273}212} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{206}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{ECF5E7}250} &
  \cellcolor[HTML]{E7F2E0}244 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_30}} &
  30 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{2281}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{ADE2BC}2804} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{77D59E}2642} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}3646} &
  \cellcolor[HTML]{F7FAF5}3466 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1119} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{62D093}915} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{858}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{62D093}915} &
  \cellcolor[HTML]{00B85C}\textbf{858} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}491} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{0FBB64}322} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{316}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{A5E0B8}380} &
  \cellcolor[HTML]{95DCAF}374 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qft\_50}} &
  50 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{41C780}6348} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E4F0DC}7674} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{5862}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}9236} &
  \cellcolor[HTML]{E4F0DC}7666 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}3282} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CCE9CE}2525} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1898}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{88D9A7}2315} &
  \cellcolor[HTML]{00B85C}\textbf{1898} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1324} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{0DBB63}542} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{536}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}640} &
  \cellcolor[HTML]{E2EFDA}634 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_5}} &
  5 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{37}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E7F2E1}52} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E7F2E1}52} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}62} &
  \cellcolor[HTML]{FFFFFF}62 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{13}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{13}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{13}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{13}} &
  \cellcolor[HTML]{FFFFFF}\textbf{13} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{6}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F1F7ED}35} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F1F7ED}35} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}44} &
  \cellcolor[HTML]{FFFFFF}44 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_10}} &
  10 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{162}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{A6E0B8}187} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{A6E0B8}187} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}230} &
  \cellcolor[HTML]{FFFFFF}230 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFF6EB}56} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{49}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{49}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{49}} &
  \cellcolor[HTML]{00B85C}\textbf{49} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{11}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFF6EB}94} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFF6EB}94} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}124} &
  \cellcolor[HTML]{FFFFFF}124 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_30}} &
  30 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{530}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{BAE5C3}637} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{BAE5C3}637} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}790} &
  \cellcolor[HTML]{FFFFFF}790 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F8F0}185} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{169}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{169}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{169}} &
  \cellcolor[HTML]{00B85C}\textbf{169} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{26}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFF6EB}274} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFF6EB}274} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}364} &
  \cellcolor[HTML]{FFFFFF}364 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_80}} &
  80 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1545}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{98DDB0}1762} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{98DDB0}1762} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F0F7EC}2190} &
  \cellcolor[HTML]{F0F7EC}2190 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}559} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{469}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{469}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{469}} &
  \cellcolor[HTML]{00B85C}\textbf{469} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{63}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFF6EB}721} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EFF6EB}721} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}960} &
  \cellcolor[HTML]{FFFFFF}960 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{grover\_diff\_100}} &
  100 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1936}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{99DDB1}2212} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{99DDB1}2212} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2750} &
  \cellcolor[HTML]{FFFFFF}2750 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}695} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{589}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{589}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{589}} &
  \cellcolor[HTML]{00B85C}\textbf{589} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{78}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}901} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}901} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1200} &
  \cellcolor[HTML]{FFFFFF}1200 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_5\_linear\_20}} &
  5 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F2F8EF}341} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{326}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{326}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}345} &
  \cellcolor[HTML]{FFFFFF}345 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8FBF6}93} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{80}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{80}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{80}} &
  \cellcolor[HTML]{00B85C}\textbf{80} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}114} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{106}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{106}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{106}} &
  \cellcolor[HTML]{00B85C}\textbf{106} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_5\_circular\_20}} &
  5 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}473} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{405}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{405}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{405}} &
  \cellcolor[HTML]{00B85C}\textbf{405} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}184} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{100}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{100}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{100}} &
  \cellcolor[HTML]{00B85C}\textbf{100} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{221}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}222} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}222} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}222} &
  \cellcolor[HTML]{E2EFDA}222 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_5\_full\_20}} &
  5 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{326}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{8FDAAB}446} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{8FDAAB}446} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}705} &
  \cellcolor[HTML]{FFFFFF}705 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{85}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}200} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}200} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}200} &
  \cellcolor[HTML]{FFFFFF}200 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{111}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{61CF92}144} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{61CF92}144} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}264} &
  \cellcolor[HTML]{FFFFFF}264 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_10\_linear\_40}} &
  10 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1591} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1451}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1451}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{7DD6A2}1490} &
  \cellcolor[HTML]{7DD6A2}1490 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}480} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{360}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{360}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{360}} &
  \cellcolor[HTML]{00B85C}\textbf{360} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}277} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{216}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{216}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{216}} &
  \cellcolor[HTML]{00B85C}\textbf{216} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_10\_circular\_40}} &
  10 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}4348} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1610}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1610}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1610}} &
  \cellcolor[HTML]{00B85C}\textbf{1610} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1749} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{400}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{400}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{400}} &
  \cellcolor[HTML]{00B85C}\textbf{400} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}924} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{842}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{842}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{842}} &
  \cellcolor[HTML]{00B85C}\textbf{842} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_10\_full\_40}} &
  10 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1592}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{8BD9A9}2891} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{8BD9A9}2891} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}5810} &
  \cellcolor[HTML]{FFFFFF}5810 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{476}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1800} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1800} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1800} &
  \cellcolor[HTML]{FFFFFF}1800 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{275}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{71D39B}489} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{71D39B}489} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1129} &
  \cellcolor[HTML]{FFFFFF}1129 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_20\_linear\_50}} &
  20 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}4065} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{3821}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{3821}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{5ACE8E}3870} &
  \cellcolor[HTML]{5ACE8E}3870 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1152} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{950}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{950}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{950}} &
  \cellcolor[HTML]{00B85C}\textbf{950} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}401} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{286}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{286}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{286}} &
  \cellcolor[HTML]{00B85C}\textbf{286} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_20\_circular\_50}} &
  20 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}20533} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{4020}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{4020}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{4020}} &
  \cellcolor[HTML]{00B85C}\textbf{4020} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}9048} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1000}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1000}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1000}} &
  \cellcolor[HTML]{00B85C}\textbf{1000} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E8F2E1}2207} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{2052}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{2052}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{2052}} &
  \cellcolor[HTML]{00B85C}\textbf{2052} \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{hea\_20\_full\_50}} &
  20 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{4063}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{93DBAE}12371} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{93DBAE}12371} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}29520} &
  \cellcolor[HTML]{FFFFFF}29520 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1147}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}9500} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}9500} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}9500} &
  \cellcolor[HTML]{FFFFFF}9500 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{401}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{80D7A3}1119} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{80D7A3}1119} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2919} &
  \cellcolor[HTML]{FFFFFF}2919 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_6\_0\_3}} &
  6 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E5F1DE}98} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{85}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{4ECB87}89} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}108} &
  \cellcolor[HTML]{FFFFFF}108 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{23}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E5F0DE}24} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E5F0DE}24} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E5F0DE}24} &
  \cellcolor[HTML]{E5F0DE}24 &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{36}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{20BF6E}37} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{20BF6E}37} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}50} &
  \cellcolor[HTML]{FFFFFF}50 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_6\_0\_6}} &
  6 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{3EC77E}97} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{93}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{93}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}122} &
  \cellcolor[HTML]{FFFFFF}122 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{25}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EEF5E9}28} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EEF5E9}28} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EEF5E9}28} &
  \cellcolor[HTML]{EEF5E9}28 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{37}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{A2DFB6}51} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{A2DFB6}51} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}76} &
  \cellcolor[HTML]{FFFFFF}76 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_17\_0\_3}} &
  17 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{41C780}432} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{406}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{406}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}586} &
  \cellcolor[HTML]{FFFFFF}586 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{148}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{148}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{148}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{148}} &
  \cellcolor[HTML]{FFFFFF}\textbf{148} &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{7BD5A0}90} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{81}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{81}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}114} &
  \cellcolor[HTML]{FFFFFF}114 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_17\_0\_6}} &
  17 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{731}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{1CBF6C}761} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{1CBF6C}761} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1202} &
  \cellcolor[HTML]{FFFFFF}1202 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{253}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E3EFDB}324} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E3EFDB}324} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E3EFDB}324} &
  \cellcolor[HTML]{E3EFDB}324 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{128}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{7DD6A1}161} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{7DD6A1}161} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}247} &
  \cellcolor[HTML]{FFFFFF}247 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_28\_0\_3}} &
  28 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{31C477}1007} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{952}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{952}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E3EFDB}1456} &
  \cellcolor[HTML]{E3EFDB}1456 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{356}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}384} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}384} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDA}384} &
  \cellcolor[HTML]{E2EFDA}384 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{151}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{1EBF6D}156} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{1EBF6D}156} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}225} &
  \cellcolor[HTML]{FFFFFF}225 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_28\_0\_6}} &
  28 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1746}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{2AC273}1870} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{2AC273}1870} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E6F1DF}3052} &
  \cellcolor[HTML]{E6F1DF}3052 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{660}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E7F2E1}840} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E7F2E1}840} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E7F2E1}840} &
  \cellcolor[HTML]{E7F2E1}840 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{248}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{4DCA87}278} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{4DCA87}278} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}423} &
  \cellcolor[HTML]{FFFFFF}423 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_40\_0\_3}} &
  40 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{31C477}2169} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{2035}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{2035}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E6F1DF}3254} &
  \cellcolor[HTML]{E6F1DF}3254 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{865}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDB}884} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDB}884} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E2EFDB}884} &
  \cellcolor[HTML]{E2EFDB}884 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{251}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{4BCA86}279} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{4BCA86}279} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}418} &
  \cellcolor[HTML]{FFFFFF}418 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\multicolumn{1}{|c|}{\textbf{qaoa\_maxcut\_40\_0\_6}} &
  40 &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{3456}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{3FC77F}3876} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{3FC77F}3876} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F7FAF5}6460} &
  \cellcolor[HTML]{F7FAF5}6460 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{1361}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F1F7ED}1800} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F1F7ED}1800} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F1F7ED}1800} &
  \cellcolor[HTML]{F1F7ED}1800 &
   &
  \multicolumn{1}{c|}{\cellcolor[HTML]{00B85C}\textbf{413}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{0ABA61}418} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{0ABA61}418} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E5F0DE}629} &
  \cellcolor[HTML]{E5F0DE}629 \\ \cline{1-7} \cline{9-13} \cline{15-19} 
\end{tabular}%
}
\end{table*}

==> src/tables/counts_v4.tex <==
\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}
\begin{table*}[]
\centering
\caption{}
\label{tab:my-table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccclccccclccccc}
 &
   &
  \multicolumn{5}{c}{\textbf{Gate Count}} &
  \multicolumn{1}{c}{} &
  \multicolumn{5}{c}{\textbf{2Q Gates}} &
   &
  \multicolumn{5}{c}{\textbf{Depth}} \\
\textbf{\# qubits} &
  \textbf{Benchmark} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{PoPR}}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{qiskit -O2}}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{qiskit -O3}}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{tket\_1}}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{tket\_2}}} &
  \multicolumn{1}{c}{\textbf{}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{PoPR}}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{qiskit -O2}}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{qiskit -O3}}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{tket\_1}}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{tket\_2}}} &
  \multicolumn{1}{c}{\textbf{}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{PoPR}}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{qiskit -O2}}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{qiskit -O3}}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{tket\_1}}} &
  \STAB{\rotatebox[origin=c]{80}{\tiny{tket\_2}}} \\ \cline{3-7} \cline{9-13} \cline{15-19} 
4 &
  \multicolumn{1}{c|}{\textbf{UCCSD\_H2\_BK}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F1E783} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E4E382}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FA8A72} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{DFE282}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FB9273} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E4E382}} \\
4 &
  \multicolumn{1}{c|}{\textbf{UCCSD\_H2\_JW}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FB8F73} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CFDD81}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{D8DF81} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FCA377} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FB9B75} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D4DE81}} \\
4 &
  \multicolumn{1}{c|}{\textbf{UCCSD\_H2\_PM}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FA8D72} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F6E883}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FB9975} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FCAE79} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EAE582}} \\
12 &
  \multicolumn{1}{c|}{\textbf{UCCSD\_LiH\_BK}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FB9173} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E9E482}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FB9774} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D7DF81}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FB9D75} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{EAE582}} \\
12 &
  \multicolumn{1}{c|}{\textbf{UCCSD\_LiH\_JW}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F9766E} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E0E282}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FA8B72} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{BAD780}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FA8971} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{DEE182}} \\
12 &
  \multicolumn{1}{c|}{\textbf{UCCSD\_LiH\_PM}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F9796E} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E6E382}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FA7F70} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D0DD81}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FA8571} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E7E482}} \\
14 &
  \multicolumn{1}{c|}{\textbf{UCCSD\_BeH2\_BK}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FA8370} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E9E482}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FA8A72} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D3DE81}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FA8D72} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E9E482}} \\
14 &
  \multicolumn{1}{c|}{\textbf{UCCSD\_BeH2\_JW}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F9766E} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{DCE182}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FA8972} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{BAD780}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FA8871} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D9E081}} \\
14 &
  \multicolumn{1}{c|}{\textbf{UCCSD\_BeH2\_PM}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F9796E} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E8E482}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FA7F70} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{D5DF81}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FA8571} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{E8E482}} \\
5 &
  \multicolumn{1}{c|}{\textbf{qft\_5}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFE884} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FAE983}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{BED880} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFD981}} \\
10 &
  \multicolumn{1}{c|}{\textbf{qft\_10}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{9DCE7E} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FCB179}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{CDDC81} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FB9774}} \\
20 &
  \multicolumn{1}{c|}{\textbf{qft\_20}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{D6DF81} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FA8A72}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{7BC57C} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FECD7F} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFEB84}} \\
30 &
  \multicolumn{1}{c|}{\textbf{qft\_30}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{CEDD81} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FA8571}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{73C27B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFE583} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFEB84}} \\
50 &
  \multicolumn{1}{c|}{\textbf{qft\_50}} &
  \cellcolor[HTML]{C7DA80} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFEB84}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{FECF7F} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{6CC07B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEA84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFEB84}} \\
5 &
  \multicolumn{1}{c|}{\textbf{grover\_diff\_5}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
10 &
  \multicolumn{1}{c|}{\textbf{grover\_diff\_10}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
30 &
  \multicolumn{1}{c|}{\textbf{grover\_diff\_30}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
80 &
  \multicolumn{1}{c|}{\textbf{grover\_diff\_80}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
100 &
  \multicolumn{1}{c|}{\textbf{grover\_diff\_100}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
5 &
  \multicolumn{1}{c|}{\textbf{hea\_5\_linear\_20}} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} \\
5 &
  \multicolumn{1}{c|}{\textbf{hea\_5\_circular\_20}} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
5 &
  \multicolumn{1}{c|}{\textbf{hea\_5\_full\_20}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
10 &
  \multicolumn{1}{c|}{\textbf{hea\_10\_linear\_40}} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFEB84}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} \\
10 &
  \multicolumn{1}{c|}{\textbf{hea\_10\_circular\_40}} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} \\
10 &
  \multicolumn{1}{c|}{\textbf{hea\_10\_full\_40}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
20 &
  \multicolumn{1}{c|}{\textbf{hea\_20\_linear\_50}} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFEB84}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} \\
20 &
  \multicolumn{1}{c|}{\textbf{hea\_20\_circular\_50}} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{63BE7B}} \\
20 &
  \multicolumn{1}{c|}{\textbf{hea\_20\_full\_50}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
6 &
  \multicolumn{1}{c|}{\textbf{qaoa\_maxcut\_6\_0\_3}} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{93CB7D} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
6 &
  \multicolumn{1}{c|}{\textbf{qaoa\_maxcut\_6\_0\_6}} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
17 &
  \multicolumn{1}{c|}{\textbf{qaoa\_maxcut\_17\_0\_3}} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
17 &
  \multicolumn{1}{c|}{\textbf{qaoa\_maxcut\_17\_0\_6}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
28 &
  \multicolumn{1}{c|}{\textbf{qaoa\_maxcut\_28\_0\_3}} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
28 &
  \multicolumn{1}{c|}{\textbf{qaoa\_maxcut\_28\_0\_6}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
40 &
  \multicolumn{1}{c|}{\textbf{qaoa\_maxcut\_40\_0\_3}} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\
40 &
  \multicolumn{1}{c|}{\textbf{qaoa\_maxcut\_40\_0\_6}} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} &
  \multicolumn{1}{l|}{} &
  \cellcolor[HTML]{63BE7B} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{FFEB84} &
  \cellcolor[HTML]{F8696B} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F8696B}} \\ \cline{3-7} \cline{9-13} \cline{15-19} 
\end{tabular}%
}
\end{table*}

==> src/tables/ctpp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\caption{Compilation Performance-Time Product (CPTP) for each framework/benchmark combination}
\label{tab:ctpp}
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{framework} &
  \textbf{UCCSD} &
  \textbf{QFT} &
  \textbf{Grover Diffusion} &
  \textbf{HEA} &
  \textbf{QAOA} \\ \hline
\textbf{PoPR} &
  \cellcolor[HTML]{63BE7B}0.89 &
  \cellcolor[HTML]{63BE7B}0.71 &
  \cellcolor[HTML]{63BE7B}0.75 &
  \cellcolor[HTML]{FFEB84}0.77 &
  \cellcolor[HTML]{FFE699}0.76 \\ \hline
\textbf{qiskit -O2} &
  \cellcolor[HTML]{FFEB84}0.54 &
  \cellcolor[HTML]{FEE983}0.65 &
  \cellcolor[HTML]{85C87D}0.74 &
  \cellcolor[HTML]{63BE7B}0.82 &
  \cellcolor[HTML]{63BE7B}0.78 \\ \hline
\textbf{qiskit -O3} &
  \cellcolor[HTML]{FCB77A}0.45 &
  \cellcolor[HTML]{9FD07F}0.69 &
  \cellcolor[HTML]{FEE783}0.68 &
  \cellcolor[HTML]{AAD380}0.79 &
  \cellcolor[HTML]{DBDD92}0.77 \\ \hline
\textbf{tket\_1} &
  \cellcolor[HTML]{86C87D}0.82 &
  \cellcolor[HTML]{FFEB84}0.65 &
  \cellcolor[HTML]{FFEB84}0.69 &
  \cellcolor[HTML]{FDCF7E}0.62 &
  \cellcolor[HTML]{FDCF90}0.64 \\ \hline
\textbf{tket\_2} &
  \cellcolor[HTML]{F8696B}0.32 &
  \cellcolor[HTML]{F8696B}0.22 &
  \cellcolor[HTML]{F8696B}0.13 &
  \cellcolor[HTML]{F8696B}0.07 &
  \cellcolor[HTML]{F8696B}0.09 \\ \hline
\end{tabular}%
}
\end{table}

==> src/tables/pcoast_ft.tex <==
\begin{table}
\centering
\caption{Total gate count results from fine-tuning PCOAST's cost function. The first two columns record the best results obtained from scanning C values in the range $[0,4]$. The columns for qiskit and \tket show the best achieved result for each framework}
\label{tab:pcoast_ft}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{benchmark} & \textbf{PCOAST -C} & \textbf{PCOAST -C -r} & \textbf{PCOAST} & \textbf{qiskit} & \textbf{\tket} \\ \hline
\textbf{qft\_20}                & 868           & \textbf{648}  & 922   & 1179          & 1541          \\ \hline
\textbf{qft\_30}                & 1688          & \textbf{1283} & 2281  & 2642          & 3466          \\ \hline
\textbf{qft\_50}                & 3972          & \textbf{3153} & 6348  & 5862          & 7666          \\ \hline
\textbf{hea\_5\_circular\_20}   & 459           & \textbf{381}  & 473   & 405           & 405           \\ \hline
\textbf{hea\_5\_full\_20}       & 318           & \textbf{307}  & 326   & 446           & 705           \\ \hline
\textbf{hea\_10\_linear\_40}    & 1497          & \textbf{1412} & 1591  & 1451          & 1490          \\ \hline
\textbf{hea\_10\_circular\_40}  & 4163          & 2708          & 4348  & \textbf{1610} & \textbf{1610} \\ \hline
\textbf{hea\_10\_full\_40}      & 1514          & \textbf{1412} & 1592  & 2891          & 5810          \\ \hline
\textbf{hea\_20\_linear\_50}    & 3869          & \textbf{3772} & 4065  & 3821          & 3870          \\ \hline
\textbf{hea\_20\_circular\_50}  & 8908          & 4759          & 20533 & \textbf{4020} & \textbf{4020} \\ \hline
\textbf{hea\_20\_full\_50}      & 3887          & \textbf{3772} & 4063  & 12371         & 29520         \\ \hline
\textbf{qaoa\_maxcut\_17\_0\_3} & \textbf{381}  & 394           & 432   & 406           & 586           \\ \hline
\textbf{qaoa\_maxcut\_17\_0\_6} & \textbf{665}  & 676           & 731   & 761           & 1202          \\ \hline
\textbf{qaoa\_maxcut\_28\_0\_3} & \textbf{887}  & 912           & 1007  & 952           & 1456          \\ \hline
\textbf{qaoa\_maxcut\_28\_0\_6} & \textbf{1657} & 1667          & 1746  & 1870          & 3052          \\ \hline
\textbf{qaoa\_maxcut\_40\_0\_3} & \textbf{1894} & 1921          & 2169  & 2035          & 3254          \\ \hline
\textbf{qaoa\_maxcut\_40\_0\_6} & 3272          & \textbf{3229} & 3456  & 3876          & 6460          \\ \hline
\end{tabular}%
}
\end{table}
